LBP: Robust Rate Adaptation Algorithm for SVC Video Streaming

Video streaming today accounts for up to 55\% of mobile traffic. In this paper, we explore streaming videos encoded using Scalable Video Coding scheme (SVC) over highly variable bandwidth conditions such as cellular networks. SVC's unique encoding scheme allows the quality of a video chunk to change incrementally, making it more flexible and adaptive to challenging network conditions compared to other encoding schemes. Our contribution is threefold. First, we formulate the quality decisions of video chunks constrained by the available bandwidth, the playback buffer, and the chunk deadlines as an optimization problem. The objective is to optimize a novel QoE metric that models a combination of the three objectives of minimizing the stall/skip duration of the video, maximizing the playback quality of every chunk, and minimizing the number of quality switches. Second, we develop Layered Bin Packing (LBP) Adaptation Algorithm, a novel algorithm that solves the proposed optimization problem. Moreover, we show that LBP achieves the optimal solution of the proposed optimization problem with linear complexity in the number of video chunks. Third, we propose an online algorithm (online LBP) where several challenges are addressed including handling bandwidth prediction errors, and short prediction duration. Extensive simulations with real bandwidth traces of public datasets reveal the robustness of our scheme and demonstrate its significant performance improvement as compared to the state-of-the-art SVC streaming algorithms. The proposed algorithm is also implemented on a TCP/IP emulation test bed with real LTE bandwidth traces, and the emulation confirms the simulation results and validates that the algorithm can be implemented and deployed on today's mobile devices.

==> dingbat.tex <==
\nopagenumbers


\font\ding dingbat scaled 1200

\setbox0=\hbox{\ding\char'141}
\newdimen\charwidth \charwidth\wd0
\def\updoublerulefill{\xleaders\hbox to 10pt
            {\hss\ding\char'142 \hss}\hfill}
\def\downdoublerulefill{\xleaders\hbox to 10pt
            {\hss\ding\char'147 \hss}\hfill}
\def\leftdoublerulefill{\xleaders\vbox to 10pt
        {\vss\hbox{\ding\char'144}\vss}\vfill}
\def\rightdoublerulefill{\xleaders\vbox to 10pt
        {\vss\hbox{\ding\char'145}\vss}\vfill}

\newdimen\Width \newdimen\Height
\Width\hsize \Height\vsize
\def\rramec{\vbox to\Height
  {\hbox to\Width{\ding\char'141\updoublerulefill{\char'143}}
   \xleaders\vbox to 10pt
      {\vss\hbox to\Width{\ding\char'144\hfill\char'145}\vss}
    \vfill
    \hbox to\Width{\ding\char'146\downdoublerulefill{\char'150}}}}

\def\RRamec #1{\setbox0=\vbox{#1}\Height\ht0\advance\Height\dp0
        \Width\wd0 \advance\Width 2\charwidth 
  \vbox
  {\hbox to\Width{\ding\char'141\updoublerulefill{\char'143}}
    \hbox to\Width{\vbox to\Height{\leftdoublerulefill}\hss
    \box0\hss\vbox to\Height{\rightdoublerulefill}}
    \hbox to\Width{\ding\char'146\downdoublerulefill{\char'150}}}}

\rramec
\tolerance 800
\RRamec{\hsize 5cm Hip hip hurrahhh Hip hip hurrahhh Hip hip
hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip
hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh
Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip
hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip
hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh
Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip
hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip
hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh Hip hip hurrahhh}



\bye


==> nonrealtime_algo.tex <==
\section{Non real time streaming algorithm}
In this section, we will describe the algorithm for non-real time streaming assuming that we non-causally know the future bandwidth. We will further relax the assumption to consider prediction errors, and give an online algorithm. 

\subsection{Non-causal Algorithm}

The main difference between the real-time and non-real time streaming is that rather than skipping a frame, we will continue downloading the frame till it is downloaded. Since the main objective is to minimize the number of stalls, we consider the algorithm where there is no stall and all the delay is in the form of a start-up delay. Using the greedy policy for a certain start-up delay, we can know whether the set of frames for which base layer is downloaded, $I$, contains all the frames or not. The start-up delay is chosen as the minimum such time for which all the frames at at-least the base layer can be downloaded. This startup delay can be found by a binary search algorithm. Having found such startup delay, the real-time non-causal algorithm is used to find qualities for each of the frame.


  \subsection{Non-Real Time Scheduling with Prediction Error}
  
In the presence of certain prediction error (assuming that the the error has zero mean), we use the startup delay and the schedule as decided above and start fetching the frames. However, if a frame is not completed by its deadline at the required quality and at-least base layer was received, the frame is played at the largest possible quality and we continue forward. However, if the current frame is not downloaded by its deadline even in the base layer, a re-optimization is performed at that point to find the startup delay for the future time bin such that there is no expected stall. We note that the adjustments of random dropping an random increase as mentioned for real-time streaming can also be used in this case.



\subsection{Non-Real Time Online Scheduling Algorithm}

We assume that the optimization is performed very $\alpha$ time-instants and the prediction for a window of length $W$ is known. We first assume that the bandwidth is known perfectly. Assuming the bandwidth for the next $W$ time-instants, the proposed non-causal optimization algorithm is performed (including finding a startup delay needed, if any) for all the frames that have not been downloaded so far and are within the first $W-d$ time instants of this window. If these frames are downloaded earlier, the rest of the frames are downloaded in the highest quality.

In the presence of prediction error, similar modifications are made as in the previous subsection. More precisely, the part of the frame not downloaded by its deadline is skipped. If the base layer is not downloaded by its deadline, we re-start the $W$ length interval at this point and thus re-compute the decisions for the next $W$ time-instants at this point .The random drop and random increase policies are also utilized for the schedule till the $W-d$ frames.

==> nonrealtime_sims.tex <==
\section{Non real time simulation and results}
        We start with a scenario we created where we simulated a video of 20 minute length using the bandwidth profile shown in Fig. \ref{fig:nonRealToy}. We compared our online SVC, $W=120$, $\alpha=60$, $PE= 20\%$ with Netflix BBA-0 algorithm which is described on [2]. \\
        It is clearly shown from the figure that online SVC delivers frames in higher average play rate than BBA-0. Average play rate of SVC is 1.48Mbps while it is 1.0 Mbps for BBA-0.\\
        BBA-0 is buffer based algorithm. It does not really predict the bandwidth, and that is why we see from figure() it does not start delivering frames in $1^st$ enhancement layer at the beginning. It takes it more than 8 minutes to reach the point in the buffer where the algorithm decides to fetch frames in higher layer. However, because the bandwidth is varying in a way peak-trough-peak, we see that even after the algorithm starts fetching higher layer, it keep oscillating between base and 1st enhancement layer. In other hand, SVC starts this oscillation process very early, thanks to the prediction. It takes the advantage of the peak to fetch frames in highest possible quality considering not to run into stalls in frames corresponding to trough time.
 \begin{figure*}
\centering
\epsfig{file=figures/bw_cos_1200s.eps, height=2in, width=3in}
\epsfig{file=figures/playRate_svc_vs_netflix_cos_f_60.eps, height=2in, width=3in}
\caption{Non real time toy example, (a) Bandwidth profile, and (b) Playback rate}
\label{fig:nonRealToy}
\end{figure*}

\subsection{Non real time real scenarios}
We compared our online algorithm ($W=120$, and $\alpha=20$, $ PE=20\%$) with BBA-0 algorithm in some real collected bandwidth profiles. We used bandwidth profile 3 with average bandwidth of 2.5, and bandwidth profile 4 with average bandwidth of 3, and 2Mbps. 3Mbps looks  high, but actaully the high bandwidth regime comse very late. It is at the end of the video time.
In the case of bandwidth profile 3 with average 2.5Mbps, as shown in Fig. \ref{fig:nonRealbw1}, SVC starts fetching frames in the quality of the highest enhancement layer immidiatlly and it continues delivering frames on this quality level, while it took the BBA0 algorithm about 250s to reach the highest enhancement layer. The reason is that the average bandwidth is high and BBA0 is waiting to fill the buffer up to $B \geq B_{min}$ $(90)$ beforeit starts  fetching frames inquality of higher enhancement layer, and up to $B \geq B_m$ $(120)$ to deliver frames in highest quality level. Average delivering quality of SVC is 2.03Mbps, and average delivering quality of BBA-0 is 1.6Mbps

 \begin{figure}
\centering
\epsfig{file=figures/playback_svc_W_120_alpha_20_avg_bw_c_25_z_800_delay_0_20_percent_prediction_error_vs_netflix.eps, height=2in, width=3in}
\caption{Playback rate of non real svc vs netflix BBA-0, for bandwidth profile 3 with average BW of 2.5Mbps}
\label{fig:nonRealbw1}
\end{figure}

In the case of bandwidth profile 3 with average 1.5Mbps, as shown in Fig. \ref{fig:nonRealbw1_15}, SVC starts fetching frames in the quality of the highest enhancement layer immidiatlly and it continues delivering frames on this quality level, while it took the BBA0 algorithm about 250s to reach the highest enhancement layer.However, close to the end the bandwidth is running very low, so SVC algorithm run into many stalls.It took it 74 more seconds to finish delivering all frames. It is expected when the window size is small, average bandwidth is low, and the good regime comes first to see stalls when bandwidth run low later. Average delivering quality of SVC is 1.7Mbps, and average delivering quality of BBA-0 is 1.45Mbps

 \begin{figure}
\centering
\epsfig{file=figures/playback_svc_W_120_alpha_20_avg_bw_c_155_z_800_delay_74_20_percent_prediction_error_vs_netflix.eps, height=2in, width=3in}
\caption{Playback rate of non real svc vs netflix BBA-0, for bandwidth profile 3 with average BW of 1.5Mbps}
\label{fig:nonRealbw1_15}
\end{figure}

In profile 4 with average bandwidth of 3Mbps, the bandwidth starts very low at the beginning and it gets much higher at the end. As the Fig. \ref{fig:nonRealbw2_3} shows, since the bandwidth is very low at the begining both algorithms continue fetching frames at the base layer quality. However, close to the end the bandwidth improves significantly. Therefore, SVC instantainuosly takes advantage of the bandwidth improvement and delivers the remaining frames at thehighest possible quality. In the contrast to that, BBA-0 continue buffering frames and it does not move to fetching higher layers until very late where almost the video reached its end. The average quality of SVC is 1.7Mbps while the average quality of BBA-0 is 1.12Mbps.
 \begin{figure}
\centering
\epsfig{file=figures/bw2_playback_svc_W_120_alpha_20_avg_bw_c_3_z_700_delay_0_20_percent_prediction_error_vs_netflix.eps, height=2in, width=3in}
\caption{Playback rate of non real svc vs netflix BBA-0, for bandwidth profile 4 with average BW of 3Mbps}
\label{fig:nonRealbw2_3}
\end{figure}

In profile 4,with average bandwidth of 1.9 Mbps. As the Fig. \ref{fig:nonRealbw2} shows, netflix finish fetching frames sooner than SVC in the cost of lower quality. Moreover, we can see that both algorithms run into stalls in the play back because of the low bandwidth at the beginning. The total amount of time interruptions for SVC is little bit higher than netflix with values of 41 and 30 respectively. However, SVC was able to deliver about $40\%$ of the frames on a quality of $1^{st}$ enhancement layer or more while netflix algorithm fetche all frames in base layer quality.
 \begin{figure}
\centering
\epsfig{file=figures/bw2_playback_svc_W_120_alpha_20_avg_bw_c_2_z_700_delay_41_20_percent_prediction_error_vs_netflix.eps, height=2in, width=3in}
\caption{Playback rate of non real svc vs netflix BBA-0, for bandwidth profile 4 with average BW of 2Mbps}
\label{fig:nonRealbw2}
\end{figure}



==> proofs.tex <==
\section{Appendix A: Proof of Lemma 4.1}
Assume running backward algorithm for $n$th layer ($n \geq 0$). According to backward algorithm $n$th layer of chunk $i_s$ is skipped in three scenarios:\\
\begin{itemize}
\item First, When layer $n-1$ of the chunk $i_s$ is not fetched. Otherwise, constraint (\ref{equ:c2eq1}) will be violated. Mathematically, when $Z_{n-1,{i_s}}=0$.
\item Secondly, when after removing whatever reserved to fetch other chunks, the bandwidth from the lower to the higher deadline of chunks $i_s$ $(t(i_s)\quad to \quad deadline(i_s))$ is not enough to fetch chunk $i_s$ up to $n$th layer quality. Mathematically:
\begin{equation}
 a(i_s)+\sum_{j=t(i_s)+1}^{(i_s-1)L+s}B(j) - \sum_{i^\prime>i_s}\sum_{j=t(i_s)}^{(i_s-1)L+s}(x(i^\prime,j)) < X_{n-1}+Y_{n}
 \end{equation}
Where, $i^\prime \in \{i_s+1,.....,C\}, i^\prime \neq i$, $X_{n-1}=\sum_{n=0}^{n-1}Y_n$, and $x(i^\prime,j)$ is the fetching policy of chunks $> i_s$.

\item Third, when chunks $i_s$ to $i_e$ (excluding the skipped chunks in between) need to be in the buffer at a certain time (i.e. $t(i_e) < deadline (i_s)$) in order not to skip $n$th layer of $i_s$, but their length is longer than the buffer duration. Mathematically there is a segment of chunks, $I=\{i_s,.....,i_e\}$  with length $N=i_e-i_s+1- \sum_{i_s}^{i_e} {\bf1}\{ Z_0(i)=0\} $, such that:
 \begin{equation}
N \cdot L > B_m
 \end{equation}
 \end{itemize}
 
 %\begin{equation}
% \sum_{j=t(i)}^{j=(i_e-1)L+s}\sum_{i=i_s}^{i_e}x(i,j) \geq N\cdot X_0 \ \text{and} \quad N \cdot L > B_m
% \end{equation}
% \end{itemize}
 %Skipping any of them is fine in term of reducing the number of skips since skipping any of them is one chunk skip. %However, for the same reason in (i) skipping $i_s$ is the one that maximizes the number of candidates to the next layer, hence skipping $i_s$ is the optimal choice, and that concludes the proof.
 First of all, For first scenario, we clearly see that any algorithm has to skip $n$th layer of chunk $i_s$. Otherwise, the solution will not be feasible.\\
 Secondly we clearly see in both $2$nd and $3$rd scenarios, there should be a skip for $n$th layer of a chunk $i$ such that $ i_s \leq i \leq min(i_e,i^{\prime\prime},C)$ where $i^{\prime\prime}$ is the nearest $n$th layer skip in the ascending order; otherwise either the buffer or the bandwidth constraint is violated.\\
  However the decision is $n$th layer of which chunk need to be skipped. It does not need to be skipping the $n$th layer of $i_s$ in order to satisfy the constraints. However, the skip that maximizes the $n$th layer objective is the optimal choice.
 
 If $i_s$ is the one that is skipped, then the objective is:
\begin{equation}
f_s=\sum_{i=1}^{i_s-1}\beta^i Z_{n,i}+\sum_{i=i_s+1}^{C}\beta^i Z_{n,i}
\label{equ:eq1_objective}
\end{equation}

If $i^\prime > i_s$ is skipped , then the objective is: 
\begin{equation}
f^\prime=\sum_{i=1}^{i^\prime-1}\beta^i Z_{n,i}+\sum_{i=i^\prime+1}^{C}\beta^i Z_{n,i}
\label{equ:eq1_objective}
\end{equation}

 
 To prove that backward algorithm choice is optimal, Let's:\\
 First, assume that there is another algorithm that achieves higher objective by skipping $n$th layer of chunk $i^\prime  > i_s$.\\
 We know that since chunks are fetched in sequence (in order), the following must hold.
 
 $t(i_s) \leq t(i^\prime)$\\
% Since skipping any of them makes the constraints non violated, then the one that maximizes the $n$th layer objective is the optimal choice.
Now, let's define the following:\\
$i_t=min(i_e,i^{\prime\prime},C)$.\\
$i_d=i$, such that, $deadline(i)=t(i_s)$. The index of the chunk with deadline$=t(i_s)$.\\
$i_k=i$, such that, $deadline(i)=t(i^\prime)$. The index of the chunk with deadline$=t(i^\prime)$.\\
%${\bf 1(.)}$: indicator function, has value 1 if $(.)$ is true, and 0 otherwise.\\

 Since $t(i_s) \leq t(i^\prime)$, we have $i_d \leq i_s  < i^\prime$. However, $i_k$ could be lower or higher than $i_s$.\\
 %The $n$th layer objective function is:
 %\begin{align*}
%f_n=\sum_{i=1}^C Z_{n,i}
%\label{equ:eq1_objective}
%\end{align*}
What can be Fetched of $n$th layer for all chunks can be expressed as following: 
 \begin{align*}
&g_n=\sum_{i=1}^C\sum_{j=1}^{deadline(C)}z_n(i,j)\\&=\sum_{i=1}^{i_d}\sum_{j=1}^{t(i_s)}z_n(i,j)+\sum_{i=i_d+1, i \neq i_s}^{i_k}\sum_{j=t(i_d)}^{t(i^\prime)}z_n(i,j)\\&+\sum_{i=i_k+1, i \neq (i_s,i^\prime)}^{i_t}z_n(i,j)+\sum_{j=t(i_s)}^{deadline(i_s)}z_n(i_s,j)+\sum_{j=t(i^\prime)}^{deadline(i^\prime)}z_n(i^\prime,j)
%\label{equ:eq1_objective}
\end{align*}
%+\sum_{j=t(i^\prime)}^{deadline(i^\prime)}z_n(i^\prime,j)
However, we already know that  $\sum_{j=t(i^\prime)}^{deadline(i^\prime)}z_n(i^\prime,j)=Y_n$. Otherwise, $i^\prime$ is not a candidate for $n$th layer, hence we can't choose to skip its $n$th layer.\\
Let:\\
$\eta= \sum_{j=t(i_s)}^{deadline(i_s)}z_n(i_s,j)$.\\  %and $\gamma_2=\sum_{j=t(i^\prime)}^{deadline(i^\prime)}z_n(i^\prime,j)$.\\
 
$g_n^{1}=\sum_{i=1}^{i_d-1}\sum_{j=1}^{t(i_s)-1}z_n(i,j)$, and $g_n^{2}=\sum_{i=i_d, i \neq i_s}^{i_k-1}\sum_{j=t(i_d)}^{t(i^\prime)-1}z_n(i,j)$.\\

$g_n^{3}=\sum_{i=i_k, i \neq (i_s,i^\prime)}^{i_t}z_n(i,j)+\eta+Y_{n}$.\\

Skipping $n$th layer of $i_s$ would free up $\eta Mb$, and Skipping $i^\prime$ would free up $Y_{n} Mb$.\\
Now, let's define:\\
 $g_n^s$: total fetched when $n$th layer of $i_s$ is skipped.\\
 $g_{n,i_s}^1$, $g_{n,i_s}^2$, and $g_{n,i_s}^3$, as $g_n^1$, $g_n^2$, and $g_n^3$ respectively when $n$th layer of $i_s$ is skipped.\\
Similarly for $i^\prime$:\\
$g_n^\prime$: total fetched when $n$th layer of $i^\prime$ is skipped.\\
 $g_{n,i^\prime}^1$, $g_{n,i^\prime}^2$, and $g_{n,i^\prime}^3$, as $g_n^1$, $g_n^2$, and $g_n^3$ respectively when $n$th layer of $i^\prime$ is skipped.
 
 %First, when $\gamma < Y_{n}$, skipping $n$th layer of $i_s$ yields: 
 %$g_n^s \geq g_n^\prime$, and
  %$f_s \geq f^\prime$. for any $\beta \geq 1$\\
 %which contradict the assumption.
 
 %Secondly, When $\gamma \geq Y_n$\\
Whatever freed up by skipping $i^\prime$ can't be used to fetch $n$th layer of chunks with indices $< i_k$ because their deadlines are earlier than $t(i^\prime)$. Therefore, we start with the case when whatever freed up by either skipping $n$th layer of $i_s$ or $i^\prime$ is used by chunks $> i_k$, then we clearly see that:\\
$g_{n,i_s}^{3}=g_{n,i^\prime}^{3}$, which yields:\\
$g_n^{s}=g_n^{\prime}$.\\
 Therefore, for $\beta = 1$, skipping any of them would yield same $n$th layer objective.\\
  However, for $\beta > 1$, skipping $i_s$ would yield higher objective since:

$\beta^{i_s} Z_{n,i_s} < \beta^{i^\prime} Z_{n,i^\prime}$, yields:

$f^\prime < f_s$.\\
 which contradict the assumption.

Secondly, if chunks $> i_k$ are fetched up to their highest possible quality, and there is still remaining $\alpha_1 \leq \eta$ in case of skipping $i_s$, or $\alpha_2 \leq Y_n$ in case os skipping $i^\prime$.

We clearly see that non of $\alpha_1$ and $\alpha_2$ can be used to fetch $n$th layer of chunks $<i_d$ since what they free up is after the deadline of those chunks. Therefore $g_n^{1}=g_{n,i_s}^1=g_{n,i^\prime}^1$. However, $\alpha_1$ can be used to increase $g_n^{s,2}$ since chunks $i_d$ to $i_k-1$ have their deadlines after $\geq t(i_s)$, but $\alpha_2$ can't be used to fetch $n$th layer of chunks $<i_k$ since they have earlier deadlines than $t(i^\prime)$. Therefore;\\

$$g_{n,i_s}^{2}=\sum_{i=i_d, i \neq i_s}^{i_k-1}\sum_{j=t(i_d)}^{t(i^\prime)-1}z_n(i,j)+\alpha_1 \geq g_{n,i^\prime}^{2}=\sum_{i=i_d, i \neq i_s}^{i_k-1}\sum_{j=t(i_d)}^{t(i^\prime)-1}z_n(i,j)$$


This yields:\\

$g_n^\prime \leq g_n^s$, which yields:\\

$f^\prime < f_s$, for $\beta \geq 1$

Which contradict the assumption.

Hence Backward algorithm yields the maximum $n$th layer objective, and that concludes the proof.


\if 0

when $i_k > i_s$:
 \begin{align*}
&f_n=\sum_{i=1}^{i_d-1} Z_{n,i}+\sum_{i=i_d}^{i_s-1} Z_{n,i}+Z_{n,i_s}+\sum_{i=i_s+1}^{i_k-1} Z_{n,i}\\&+\sum_{i=i_k}^{i^\prime-1} Z_{n,i}+Z_{i^\prime}+\sum_{i=i^\prime+1}^{i_e} Z_{n,i}+\sum_{i=i_e+1}^{i_t} Z_{n,i}+\sum_{i=i_t+1}^{C} Z_{n,i}
%\label{equ:eq1_objective}
\end{align*}

when $i_k \leq i_s$:
 \begin{align*}
&f_n=\sum_{i=1}^{i_d-1} Z_{n,i}+\sum_{i=i_d}^{i_k-1} Z_{n,i}+\sum_{i=i_k}^{i_s-1} Z_{n,i}+Z_{n,i_s}\\&+\sum_{i=i_s+1}^{i^\prime-1} Z_{n,i}+Z_{i^\prime}+\sum_{i=i^\prime+1}^{i_e} Z_{n,i}+\sum_{i=i_e+1}^{i_t} Z_{n,i}+\sum_{i=i_t+1}^{C} Z_{n,i}
%\label{equ:eq1_objective}
\end{align*}


Skipping $n$th layer of $i_s$ or $i^\prime$ frees bandwidth of $\delta \leq Y_n Mb$, and since, chunks are fetched in sequence (in order), and no chunk can be fetched after its deadline. Skipping the $n$th layer of the one that have earlier deadline would offer more bandwidth for chunks < $i^\prime$. Mathematically,\\
If $n$th layer of $i_s$ frees $\delta=\alpha_1+\gamma_1$, where $\alpha_1$ is the bandwidth that is freed when $n$th layer of $i_s$ is skipped for the time period $j \leq deadline(i^\prime-1)$, and $\gamma_1$ is the bandwidth that is freed when $n$th layer of $i_s$ is skipped for the time period $j > deadline(i_s-1)$, and If $n$th layer of $i^\prime$ frees $\delta=\alpha_2+\gamma_2$, where $\alpha_2$ is the bandwidth that is freed when $n$th layer of $i^\prime$ is skipped for the time period $j \leq deadline(i^\prime-1)$, and $\gamma_2$ is the bandwidth that is freed when $n$th layer of $i^\prime$ is skipped for the time period $j > deadline(i^\prime-1)$.
 
$deadline(i_s) < deadline(i^\prime)$, and chunks are fetched in sequence, yields:\\
$$\alpha_1 \geq \alpha_2$$ which means that 

If $i_s$ is the one that is skipped, then the objective is:
\begin{equation}
f_s=\gamma^0(\sum_{i=1}^{i_s-1}\beta^i Z_{0,i}+\sum_{i=i_s+1}^{C}\beta^i Z_{0,i})
\label{equ:eq1_objective}
\end{equation}

If $i^\prime > i_s$ is skipped , then the objective is: 
\begin{equation}
f^\prime=\gamma^0(\sum_{i=1}^{i^\prime-1}\beta^i Z_{0,i}+\sum_{i=i^\prime+1}^{C}\beta^i Z_{0,i})
\label{equ:eq1_objective}
\end{equation}

Since $\beta > 1$, we clearly see that $f^\prime$ is less than $f_s$:
\begin{equation}
f^\prime < f_s
\end{equation}
Which contradict the assumption.


\begin{equation}
sum_{i=t(i_s)}^{i^\prime-1} Z_{n,i}+\sum_{i=i_s+1}^{C}\beta^i Z_{0,i})
\label{equ:eq1_objective}
\end{equation}

\fi


 %later chunks up to either $i^{\prime \prime}$, where $i^{\prime \prime}$ is the the last one before next skip (first case) or $i_e$ (second case) can be fetched and $\delta$ more bandwidth is available, so it can be used to fetch higher layers of chunks $i_s+1$ to $i_m=\min(i_e,i^{\prime \prime})$ and/or basel layer of chunk $i_s-1$. %Therefore, the objective is:

% \begin{equation}
%f=\gamma^0\sum_{i=1}^{i_s-1}\beta^i Z_{0,i}+\gamma^0\sum_{i=i_s+1}^{i_m}\beta^i Y_{0,i}+\gamma^0\sum_{i=m+1}^{C}\beta^i Z_{0,i}+\gamma^1\sum_{i=1}^{C}\beta^i Z_{1,i}+.....+\gamma^n\sum_{i=1}^{C}\beta^i Z_{n,i}
%\label{equ:eq1_objective}
%\end{equation}
 \if 0


\section{Appendix B: Proof of Theorem 4.4}

%
Since $\gamma \ll 0, \beta > 1$, and $\sum_{j > k}\gamma^j \sum_i\beta^i Z_{j,i} \ll \gamma^k \beta Z_{k,1}$, then, the following holds for any $j > k$:\\

%\begin{equation}
%\gamma^k\beta Z_{k,1} \gg \gamma^j \beta^C Z_{j,C}
%\label{equ:eq1_objective}
%\end{equation}

\begin{equation}
\gamma^k\sum_{i=1}^{C}\beta^i Z_{k,i} \gg \gamma^j\sum_{i=1}^{C}\beta^i Z_{j,i}.
\label{equ:eq1a2}
\end{equation}

(\ref{equ:eq1a2}) implies that the algorithm that delivers more enhancement layers and less base layers can't achieve higher objective. i.e, if there is an algorithm 1 with size decisions ${\mathcal Z}^\prime$, and another one with size decisions ${\mathcal Z}^*$, such taht:\\

%if there is an  algorithm that has higher number of enhancement layers and less number of base layers than what is achieved by backward algorithm on base layer, this algorithm can't have higher objective. i.e, if:\\

\begin{equation}
\sum_{n=1}^N \gamma^n\sum_{i=1}^{C}\beta^i Z_{n,i}^\prime > \sum_{n=1}^N \gamma^n\sum_{i=1}^{C}\beta^i Z_{n,i}^*
\label{equ:eq1_objective}
\end{equation}
and
\begin{equation}
\gamma^0\sum_{i=1}^{C}\beta^i Z_{0,i}^\prime <  \gamma^0\sum_{i=1}^{C}\beta^i Z_{0,i}^*
\label{equ:eq1_objective}
\end{equation}

then:\\

\begin{equation}
\sum_{n=0}^N \gamma^n\sum_{i=1}^{C}\beta^i Z_{n,i}^\prime < \sum_{n=1}^N \gamma^n\sum_{i=1}^{C}\beta^i Z_{n,i}^*
\label{equ:eq1_objective}
\end{equation}




Lemma 4.1 shows that backward algorithm achieves optimal fetching policy when only base layer is considered. Therefore, any algorithm delivers less number of base layer can't have higher objective, so we consider only algorithms that can achieve equal number of base layers to which backward can achieve.
Proposition 1 defines the first time when chunk $i$ can be fetched according to the sizes found by running backward algorithm on base layer.

Now, given the backward decisions of the base layer, the lower bound on the fetching time of the $i$th chunk $(t(i))$, the amount that was scheduled to be fetched for chunk $i$ at time $t(i)$, $(x(i,t(i))$, and the remaining bandwidth at $t(i)$ when backward algorithm was run for base layer decisions ($e(t(i)$), , we define when we skip E1 layer of a chunk.\\
 E1 is skipped in 3 scenarios:
  \begin{itemize}
\item First, when there is a chunk $i_s$ such that its base layer is not fetched, $Z_{0,{i_s}}=0$; otherwise constraint~\ref{equ:c2eq1)} is violated.

\item Secondly, when a chunk $i_s$ was considered as a candidate for base layer quality, but it can't meet its deadline if it is fetched in higher quality:
\begin{equation}
 X_0 < \sum_{j=(t(i_s)+1)}^{(i_s-1)L+s}B(j)+x(i_s,t(i_s))+e(t(i)) - \sum_{i^\prime>i}\sum_{j=t(i)}^{(i_s-1)L+s}(x(i^\prime,j)) < X_1
 \end{equation}
 In words, when the remaining bandwidth is is less than a cumulative E1 size of chunk ($X_1=X_0+Y_1$).
\item Finally, when there is a segment of chunks, $I=\{i_s,.....,i_e\}$  with length $N=i_e-i_s+1$, such that:
 %$N*L > B_m$, and $((N-1)*L=B_m$
 \begin{equation}
 \sum_{j=1}^{j=(i_e-1)L+s}\sum_{i=i_s}^{i_e}x(i,j) = X_1+\sum_{i_s+1}^{i_e} X \ \text{and} \quad N \cdot L > B_m
 \end{equation}
 where $X \in \{X_0,X_1\}$\\
 and\\
  \begin{equation}
 \sum_{j=1}^{j=(i_e-1)L+s}\sum_{i=i_s}^{i_e}x(i,j) = X_0+\sum_{i_s+1}^{i_e} X \ \text{and} \quad N \cdot L \leq B_m
 \end{equation}
 
 In words, chunks $i_s$ to $i_e$, were considered to be fetched at least at base layer quality without violating any of the constraints, but when we run backward algorithm for E1 decisions, we find in order to have some of them at E1 quality, they need to be in the buffer at a certain time, but their total length is longer than the buffer duration.
 \end{itemize}
 %Skipping any of them is fine in term of reducing the number of skips since skipping any of them is one chunk skip. %However, for the same reason in (i) skipping $i_s$ is the one that maximizes the number of candidates to the next layer, hence skipping $i_s$ is the optimal choice, and that concludes the proof.
 For first scenario, any algorithm has to skip E1 of that chunk in order to avoid violating the constraints. For both second and third scenario, we clearly see that there should be a skip for E1 of a chunk $i$ such that $ i \geq i_s$; otherwise either the buffer or the bandwidth constraint is violated, but the decision is which chunk to skip. 
 
 
 To prove that our Base layer backward followed by forward, and then  E1 backward scan (BL backwrd-forward-E1 Backward)) is optimal for up to E1 layer, Let's assume that there is another algorithm that achieves higher objective by skipping E1 of a chunk $i^\prime  > i_s$.
 Since skipping any of them makes the constraints non violated, then the one that maximizes the objective is the optimal choice. The objective function is:

If we skip E1 of $i_s$ (E1 backward decision), then the objective is:
\begin{eqnarray}
f_s=\sum_{n=0}^1\gamma^n \sum_{i=1}^{i_s-1}\beta^i Z_{n,i}+\gamma^0 \beta^{i_{s}}X_{0}\nonumber \\+\gamma^0 \beta^{i^{\prime}}X_{0}+\gamma^1 \beta^{i^{\prime}}X_{1}+\sum_{n=0}^1\gamma^n \sum_{i=i_s+1\backslash i^\prime}^{C}\beta^i Z_{n,i}.
%\label{equ:eq1_objective}
\end{eqnarray}

If $i^\prime > i_s$ is skipped (any other algorithm), then the objective is: 

\begin{eqnarray}
f^\prime=\sum_{n=0}^1\gamma^n \sum_{i=1}^{i^\prime-1}\beta^i Z_{n,i}+\gamma^0 \beta^{i_{s}}X_{0}\nonumber \\+\gamma^1 \beta^{i_{s}}X_{1}+\gamma^0 \beta^{i^{\prime}}Y_{0}+\sum_{n=0}^1\gamma^n \sum_{i=i^\prime+1}^{C}\beta^i Z_{n,i}.
%\label{equ:eq1_objective}
\end{eqnarray}


 
Since $\beta > 1$, we clearly see that $f^\prime$ is less than $f_s$:
\begin{equation}
f^\prime < f_s
\end{equation}
Which contradict the assumption.Therefore, Deadline and Buffer Aware Bin Packing algorithm finds optimal policy up to layer E1.
Taking this as base for E2, running backward algorithm at E2 will yield the optimal solution up to E2 since backward yields the optimal solution of the current layer given the lower bound on the fetching time of every chunk, and previous backwar-forward yields the optimal solution of all lower layers. Continuing the same manner up to the $N$th enhancement layer yields the maximum objective, thus solves the original problem optimally. 
\fi
%we will see the scenarios when E2 skip is needed. The extra scenario is that when there is a chunk did not get its E1, so it can't get E2 in order to not violate the constraints. Continuing the same manner up to enhancement layer $N$ solves the original problem optimally.
















%since $i^\prime$ could be be partially fetched before the deadline of the previous one ($i^\prime -1$), and more of it could be fetched after that. Therefore, the extra bandwidth $\delta$ when this chunk is skipped can't be all used to fetch base and higher layers of chunks with indices less than $i^\prime$. Therefore, If we define the objective when $i_s$ is skipped as $f_s$:
\if 0
\begin{equation}
f_s=\sum_n\gamma^n\sum_{i=1}^{i_s-1}\beta^i Z_{n,i}+\sum_n\gamma^n\sum_{i=i_s+1}^{C}\beta^i Z_{n,i}
\label{equ:eq1_objective}
\end{equation}
and the the objective when $i^\prime$ is skipped as $f^\prime$:
\begin{equation}
f^\prime=\sum_n\gamma^n\sum_{i=1}^{i^\prime-1}\beta^i Z_{n,i}+\sum_n\gamma^n\sum_{i=i^\prime+1}^{C}\beta^i Z_{n,i}
\label{equ:eq1_objective}
\end{equation}
We clearly see that $f^\prime$ is always upped bounded by $f_s$:
\begin{equation}
f^\prime \leq f_s
\end{equation}


\section{Appendix B: Proof of Lemma 2}

To prove it, we again assume forward algorithm in base layer decision. First, we assume that after running backward algorithm, we got set $I$ which is the set of chunks that can be fetched. We clearly see that the proof is obvious for Infinite buffer since all chunks in $I$ can be fetched one after another without worrying about buffer overflow and playback time of every chunk. Therefore, if a chunk $i \in I$ is fetched at $X_0$ size , it would be completely downloaded in faster time than if its fetched in size of $X_i > X_0$. Therefore any chunk $j \in I$ would have been fetched in its earliest time if all chunks $i \in I$ and $i < j$ were fetched at base layer quality.

The tricky part is when the buffer is finite, In this case, the buffer  occupancy over time may change, and some time slots that were not used because of buffer overflow in case of fetching base layer may be used if some chunks were fetched in higher sizes since the time when the buffer is full may be different.

Let's assume that the buffer can have up to $N$ chunks at most, and $I_s$ is a set contains the indices of the chunks that are in the buffer at time $t_j$.  These chunks could be of same or different sizes such that:
$\sum_{i \in I_s}({\bf 1}(X_i =X_ 0)) + \sum_{i \in I_s}({\bf 1}(X_i >X_0)) \leq N$
 
Now, let's consider two cases:
\begin{itemize}
\item First, when the buffer is full of base layer chunks at time $t_j$: 

(i) let's assume that chunks in $I_s$ are fetched at base layer size $X_0$ and the playback of the first chunk in the set $i_s$ is $\geq t_j$. Remember, the playback of every chunk $i \in I_s$ is $(i-1)L+s$. 

Without loss of generality, let's assume that the chunks that are in the buffer at time $t_j$ are chunks $1$ to $N$, and all chunks after $N$(i.e, $N+1,.....,C$) can be fetched. The total chunks that are buffered at the end of $t_j$ is $N_{t_{j}} \leq N+1-1=N$ and the index of the last chunk that can be fetched at $t_j$ is $N+1$. What would happen is that one chunk would have been played and at most one can be added if the bandwidth at $t_j$ $B(t_j)$ allows since more than 1 chunk would overflow the buffer. Therefore, at the end of the time slot $t_j$ there would be at most N buffered chunks with $N+1$ being the last chunk appended to the buffer. 
 
 (ii) some chunks in $I_s$ are fetched in quality higher than the base layer, $X_i > X_0$ for some $i \in I_s$, then at time $t_j$ the buffer may not be full since fetching higher layers would result in more fetching time per chunk which may lead to less chunks buffered at time $t_j$. Precisely, the number of chunks buffered at time slot $t_j$ is:
 $\sum_{i \in I_s}({\bf 1}(X_i >X_ 0)) + \sum_{i \in I_s}({\bf 1}(X_i >=X_0))=M \leq N$.
Note, that the index of the last chunk in the buffer is $M < N$. Let $K=N-M$. Then by the end of $t_j$, the number of chunks at the buffer $N_{t_{j}}  \leq M-1+K+1=N$, since chunk number 1 would have been played, and $K+1$ chunks would be the most that can be downloaded at time $t_j$, so the last chunk that can be appended to the buffer at time $t_j$ in order to have full buffer is the chunk $N+1$. Therefore, we just showed that the earliest time to fetch any chunk can't be before its earliest time if chunks in $I$ are fetched at base layer quality.

 \item Secondly, when the buffer is not full:
 Let's assume the two scenarios again for the same available bandwidth at time $t_j$.\\
 (i) All base layer: in this case there will be $M_1$ chunks at base layer quality in the buffer at time $t_j$ ($1,....,M_1$), where $M_1<N$. Let's define $K_1$ to be $N-M_1$, Then by the end of $t_j$, there will be $N_{t_{j}} \leq M_1-1+K_1+1=N$ chunks at the buffer. Chunk $1$ would have been played back and in order to have N chunks in the buffer, $K+1$ would need to be downloaded at time $t_j$, so chunk $N+1$ would have been the last chunk appended to the buffer.
 (ii)  some chunks in $I_s$ are fetched in quality higher than the base layer, $X_i > X_0$ for some $i \in I_s$, then the number of chunks buffered at time slot $t_j$ is:
 $\sum_{i \in I_s}({\bf 1}(X_i =X_ 0)) + \sum_{i \in I_s}({\bf 1}(X_i >X_0))=G \leq M_2 < M_1 < N$. Let $K_2=N-M_2$, $K_2 > K_1$. Then by the end of $t_j$, the number of chunks at the buffer $N_{t_{j}}  \leq M_2-1+K_2+1=N$, since chunk number 1 would have been played, then the last chunk that can be appended to the buffer at time $t_j$ in order to have full buffer is the chunk N+1. Therefore, we just showed the same result, chunks can't be fetched earlier than if all fetched at base layer.
 \end{itemize}

 
 \section{Appendix C: Proof of Lemma 3}

First without loss of generality we use chunk duration of $1s$. Therefore, the deadline of any chunk $i$ is $deadline(i)=i+d(i)$ and the playback time of chunk $i$ is $deadline(i)+1$. From lemma 1, we know that when chunks are all fetched in base layer, then every chunk is fetched in its earliest time possible, hence, the minimum stall duration if all chunks are fetched at base layer is the lowest bound to any other fetching policy.
Let's assume that the time slot when chunk $i+1$ is completely fetched is $j$. There are are two scenarios:\\
Scenario 1 ($j \leq deadline(i)+1$): In this case forward algorithm chooses $d(i+1)$ to be equal to $d(i)$ and $deadline(i+1)=i+1+d(i)=deadline(i)+1$, and playback of chunk $i+1$ would be $deadline(i+1)+1=deadline(i)+2$. Since $i+1$th chunk would be completely fetched by the time $deadline(i+1)$, hence there would be no stall, and if the stall duration up to chunk $i$ playback time is  $\alpha$ seconds, then the stall duration up to chunk $i+1$th playback time would be the same ($\alpha$ seconds). Let's assume that there is another algorithm that have $(d(i+1) > d(i))$ and provides same or less stall duration. Let's define $\delta=d(i+1)-d(i)$. Chunk $i$ playback slot is $deadline(i)+1$. Therefore, to avoid any stalls chunk $i+1$ should be played at time slot $deadline(i)+2$. If there is an algorithm such that $(d(i+1) > d(i))$, then chunk $i+1$ playback time would be $deadline(i)+2+\delta$ which has a stall duration of $\delta$ seconds. Therefore, it contradict the assumption that same stall duration can be maintained with $d(i+1) > d(i)$.

Scenario 2 ($j > deadline(i)+1$): then forward algorithm would choose $deadline(i+1)=j$ ($d(i+1)=j-(i+1) > d(i)$) and playback time is $j+1$. Let's re-write it as $d(i+1)=d(i)+\delta$. We clearly see that there would be stall duration of $\delta$ seconds (if chunk $i+1$ is played back at time slot $j+1$) added to the total stall duration up to chunk $i$ which we defined to be $\alpha$ seconds. Therefore, the total stall duration up to playback time of chunk $i+1$ is $(\alpha+\delta)$ seconds. Let's assume that there is an algorithm that have higher deadline ($j^\prime > j$) without introducing more stalls. since chunk $i+1$ is completely fetched at time slot $j$, then the nearest playback time to not introduce more stall duration is to play it back at time slot $j+1$. If it is played at any $j^\prime +1 > j+1$, that would increase the stall duration further and contradict the assumption. This confirms that the forward decision is the optimal in term of minimizing stall duration and concludes the proof.

\fi
 

==> proofsV2.tex <==
\section{Appendix A: Proof of Lemma 4.1}
Assume running backward algorithm for $nth$ layer ($n \geq 0$). According to backward algorithm, $n$th layer of chunk $i_s$ is skipped in three scenarios:\\
\begin{itemize}
\item First, When $(n-1)th$ layer of the chunk $i_s$ is not fetched. Otherwise, constraint (\ref{equ:c2eq1}) will be violated. Mathematically, when $Z_{n-1,{i_s}}=0$.
\item Secondly, when after removing whatever reserved to fetch lower layers of prior chunks and up to $nth$ layer of later chunks, the bandwidth from the lower to the higher deadline of chunks $i_s$ $(t(i_s)\quad to \quad deadline(i_s))$ is not enough to fetch chunk $i_s$ at $nth$ layer quality. Mathematically:
\begin{equation}
 \sum_{j=t(i_s)}^{(i_s-1)L+s}B(j) - \sum_{i^\prime \neq i_s}\sum_{j=t(i_s)}^{(i_s-1)L+s}(x(i^\prime,j)) < X_{n-1}+Y_{n}
 \end{equation}
Where, $X_{n-1}=\sum_{n=0}^{n-1}Y_n$, and $x(i^\prime,j)$ is the fetching policy of every chunk $i^\prime \neq i_s$.

\item Third, when chunks $i_s$ to $i_e$ (excluding the skipped chunks in between) need to be in the buffer at a certain time (i.e. $t(i_e) < deadline (i_s)$) in order not to skip $nth$ layer of $i_s$, but their length is longer than the buffer duration. Mathematically there is a segment of chunks, $I=\{i_s,.....,i_e\}$  with length $N=i_e-i_s+1- \sum_{i_s}^{i_e} {\bf1}\{ Z_0(i)=0\} $, such that:
 \begin{equation}
N \cdot L > B_m
 \end{equation}
 \end{itemize}
 
 %\begin{equation}
% \sum_{j=t(i)}^{j=(i_e-1)L+s}\sum_{i=i_s}^{i_e}x(i,j) \geq N\cdot X_0 \ \text{and} \quad N \cdot L > B_m
% \end{equation}
% \end{itemize}
 %Skipping any of them is fine in term of reducing the number of skips since skipping any of them is one chunk skip. %However, for the same reason in (i) skipping $i_s$ is the one that maximizes the number of candidates to the next layer, hence skipping $i_s$ is the optimal choice, and that concludes the proof.
 %First of all, For first scenario, we clearly see that any algorithm has to skip $n$th layer of chunk $i_s$. Otherwise, the solution will not be feasible.\\
 %Secondly we clearly see in both $2$nd and $3$rd scenarios, there should be a skip for $n$th layer of a chunk $i$ such that $ i_s \leq i \leq min(i_e,i^{\prime\prime},C)$ where $i^{\prime\prime}$ is the nearest $n$th layer skip in the ascending order; otherwise either the buffer or the bandwidth constraint is violated.\\
 % However the decision is $n$th layer of which chunk need to be skipped in order to maximize $n$th layer objective. Let us assume that skipping chunk $i^\prime > i_s$ leads to lower number of skips than skipping $i_s$.\\
  
  To prove that backward algorithm choice is optimal. We start from last chunk moving toward the first, and see if any other algorithm can have less number of $n$th layer skips.
  
  Starting from last chunk ($C$) moving backward, the first skip of $nth$ layer of a chunk ($i_1$) has to be a result of one of the 3 above mentioned scenarios.\\
  First, If backward algorithm skips $n$th layer of chunk ($i_1$) because ($n-1)th$ layer of that chunk is not fetched, then we clearly see that any algorithm has to skip the $n$th layer of chunk ($i_1$). Otherwise, the solution will not be feasible. Constraint (\ref{equ:c2eq1}) will be violated.\\
  Secondly we clearly see in both $2$nd and $3$rd scenarios, there should be a skip for $nth$ layer of a chunk ($i$) such that $ i_1 \leq i \leq min(i_{e1},C)$; otherwise either the buffer or the bandwidth constraint is violated. Therefore, any other algorithm must have one or more $n$th layer skips in the period $[i_1,min(i_{e1},C)]$. Hence, the first backward skip is necessary and can't be avoided, and any other algorithm has to have one or more $n$th layer skip in the period $[i_1,min(i_{e1},C)]$.
  
  Given first skip of the backward algorithm and the one or more skips for any other algorithm for the $[i_s,min(i_{e1},C)]$ period. There will be two kind of algorithms to compare with for the next skip.
  \begin{itemize}
  \item {\bf Algorithms that have only one skip in the period $[i_1,min(i_{e1},C)]$ (single skip algorithm)}. Any algorithm skips $nth$ layer of a chunk ($i > i_1$), would be able to fetch the $n$th layer of chunk ($i_1$) as far as the $nth$ layer of the skipped chunk ($i$) could have been fetched before the deadline of the $(i-1)th$ chunk; otherwise there still be another skip since whatever freed up by skipping $nth$ layer of chunk ($i$) can't be used by earlier chunks. However, any single skip algorithm can't fetch chunk ($i_1-1$) closer to its deadline than what backward algorithm can do even though they skip chunk with higher index, and the reason is that whatever freed up by skipping $nth$ layer of a chunk with higher index is used to fetch $n$th layer of $i_1$. 
  
  Second skip would follow the same way except for scenario 2 and 3 backward algorithm would skip $n$th layer of chunk ($i_2$) , in the period  $[i_2,min(i_{e2},i_1-1)]$, and since any other single skip algorithm was not able to fetch chunks ($i_1-1$) closer to its deadline than what backward algorithm was able to do, any single skip algorithm must have a skip or more in the period $[i_2,min(i_{e2},i_1-1)]$. For the next skip, we have algorithms that have one skip in both periods, and algorithms with one skip in the first period and more skips in the second period. For the algorithms that have single skip in both periods (single-single skip algorithm), we clearly can see since no algorithm can fetch chunk ($i_2-1$) closer to its deadline than backward algorithm, the scenario will repeat and their will be a corresponding skip to every backward skip. For algorithms with more skips in some periods, we discuss it in the next point.
 
  \item {\bf Algorithms that have more than one skip in the period $[i_1,min(i_{e1},C)]$ (multi-skip algorithm)}. Any multi-skip algorithm could fetch chunks with indecies $< i_1$ closer to their deadlines than what backward algorithm can do. If an algorithm have ($m$) skips in the period $[i_1,min(i_{e1},C)]$, then at most $n$th layers of other $m$ chunks can be fetched before backward algorithm reaches $m$th skip. However, if backward algorithm reaches $mth$ skip as it scans in the revers order at a chunk $i^\prime$, then we surely know all multi-skip algorithms can't fetch ($n$th) layer of chunk $i^\prime-1$ closer to its deadline since they used whatever freed up to fetch $m$ chunks belong to the period $> i^\prime$ at $nth$ layer quality, which means at best the multi skip algorithm can have same skips as backward algorithm. The same thing repeats after $i^\prime$. Therefore, the multi-skip algorithm can't achieve less number of skips than backward algorithm. The same thing applies when we assume that the multi skip period is any other priode than $[i_1,min(i_{e1},C)]$.
  \end{itemize}
  
  
   \section{Appendix B: Proof of Lemma 4.2}
  
  First, when $\beta=1$, the optimal $n$th layer decision is the one that minimizes the number of skips, and lemma 4.1 shows that backward algorithm achieves the minimum number of $n$th layer skips.


When $\beta > 1$, as proof of lemma 4.1 (Appendix A) shows, backward algorithm pushes all skips toward lower index chunks. For every backward skip, any other algorithm that do not skip the $n$th layer of the same chunk would have a skip or more for $n$th layers of chunks with higher index than the one that is skipped using backward algorithm. Mathematically, if backward algorithm skips $n$th layer of chunk $i$, any other algorithm that does not skip $n$th layer of $i$ would have corresponding skip for $n$th layer of chunk $i^\prime > i$.

Since, $\beta > 1$, then:\\

$\beta^{i^{\prime}} Z_{n,i^\prime} > \beta^i Z_{n,i}$, which yields

\begin{equation}
\sum_{i=1}^{C}\beta^i Z_{n,i}^\prime < \sum_{i=1}^{C}\beta^i Z_{n,i}^*
\label{equ:eq1_lemma1}
\end{equation}
% If $i_s$ is the one that is skipped, then the objective is:
%\begin{equation}
%f_s=\sum_{i=1}^{i_s-1}\beta^i Z_{n,i}+\sum_{i=i_s+1}^{C}\beta^i Z_{n,i}
%\label{equ:eq1_objective}
%\end{equation}

and shows that when $\beta > 1$, Backward algorithm achieves strictly higher objective than any other algorithm with different skipping pattern. This concludes the proof.
  
  
  
  
  
  
  
  
  
  
  
  
  %if the $n$th layer of that chunk is fetched before the deadline of $(i-1)$. Otherwise there still be another skip
 % We continue moving toward the first chunk.\\
  %The next skip will follow the same manner:\\
  % If $n-1$ of a chunk is not fetched, then any algorithm will skip $n$th layer of this chunk.\\
  % If scenario 2 or 3 is the case. Backward algorithm will skip $n$th layer of chunk $i_2$, so there will be 2 skips in the period $[i_2,C]$. We already know that it is either $[i_1,i_e]$ were in the buffer at same time. Therefore, $i_2$ 
   
  

% If $i_s$ is the one that is skipped, then the objective is:
%\begin{equation}
%f_s=\sum_{i=1}^{i_s-1}\beta^i Z_{n,i}+\sum_{i=i_s+1}^{C}\beta^i Z_{n,i}
%\label{equ:eq1_objective}
%\end{equation}

%If $i^\prime > i_s$ is skipped , then the objective is: 
%\begin{equation}
%f^\prime=\sum_{i=1}^{i^\prime-1}\beta^i Z_{n,i}+\sum_{i=i^\prime+1}^{C}\beta^i Z_{n,i}
%\label{equ:eq1_objective}
%\end{equation}
\if 0
Let's define what can be Fetched of $n$th layer for all chunks as following: 
 \begin{align*}
&g_n=\sum_{i=1}^C\sum_{j=1}^{deadline(C)}z_n(i,j)\\&=\sum_{i=1}^{i^\prime-1, i \neq i_s}\sum_{j=1}^{deadline(i^\prime-1)}z_n(i,j)+\sum_{i=i^\prime+1}^{C}\sum_{j=1}^{deadline(C))}z_n(i,j)\\&+\sum_{j=1}^{dadline(i_s)}z_n(i_s,j)+\sum_{j=1}^{dadline(i^\prime)}z_n(i^\prime,j)
%\label{equ:eq1_objective}
\end{align*}

 However, we already know that:\\
 $\sum_{j=1}^{deadline(i_s)}z_n(i_s,j)=\sum_{j=1}^{deadline(i^\prime)}z_n(i^\prime,j)=Y_n$. Otherwise, $i_s$ or $i^\prime$ is not a candidate for $n$th layer, hence we can't choose to skip its $n$th layer.\\
 
 Therefore, $g_n$ reduces to:\\
 \begin{align*}
&g_n=\sum_{i=1}^C\sum_{j=1}^{deadline(C)}z_n(i,j)\\&=\sum_{i=1}^{i^\prime-1, i \neq i_s}\sum_{j=1}^{deadline(i^\prime-1)}z_n(i,j)+\sum_{i=i^\prime+1}^{C}\sum_{j=1}^{deadline(C))}z_n(i,j)+2Y_n
%\label{equ:eq1_objective}
\end{align*}

Moreover, the $n$th layer objective is:\\
\begin{equation}
f_n=\sum_{i=1}^{C}\beta^i Z_{n,i}
%\label{equ:eq1_objective}
\end{equation}

Now, let:\\
$g_{n,i_s}^{1}=\sum_{i=1, i \neq i_s}^{i^\prime-1}\sum_{j=1}^{deadline(i^\prime-1)}z_n(i,j)$, and $g_{n,i_s}^{2}=\sum_{i=i^\prime+1}^C\sum_{j=1}^{deadline(C)}z_n(i,j)$ when $i_s$ is skipped.\\
Similarly:\\
$g_{n,i^\prime}^{1}=\sum_{i=1, i \neq i_s}^{i^\prime-1}\sum_{j=1}^{deadline(i^\prime)}z_n(i,j)$, and $g_{n,i^\prime}^{2}=\sum_{i=i^\prime+1}^C\sum_{j=1}^{deadline(C)}z_n(i,j)$ when $i^\prime$ is skipped.\\
Moreover, $g_{n,i_s}$, and $g_{n,i^\prime}$ as the total fetched when chunk $i_s$ and chunk $i^\prime$ skipped respectively.\\
$f_{n,i_s}$ and $f_{n,i^\prime}$ the $n$th layer objective when chunk $i_s$ and chunk $i^\prime$ skipped respectively.\\
First, we clearly see that:\\
$g_{n,i_s}^{2}=g_{n,i^\prime}^{2}$, since whatever skipping $i_s$ can give to chunks $> i^\prime$, skipping chunk $i^\prime$ can also give.\\
Therefore, When $\beta=1$
$f$
However, skipping $i^\prime$ can't help chunks $< i^\prime$ when the deadline of $i^{\prime-1}$ is before the $t(i^\prime)$. i.e when  $deadline(i^\prime-1) < t(i^\prime)$. Therefore;

$$g_{n,i_s}^{1} \geq g_{n,i^\prime}^{1}$$, yields:\\
$$g_{n,i_s} \geq g_{n,i^\prime}$$\\
Since $\beta \geq 1$. This yields:\\
$f_{n,i^\prime} \leq f_{n,i_s}$
Which contradict the assumption and proves the optimality of backward algorithm %in term of minimizing the number of skips. \\
Moreover, when $\beta$ is strictly greater than 1($\beta > 1$), $f_{n,i_s}$ is strictly greater than $f_{n,i^\prime}$ ($f_{n,i_s} > f_{n,i^\prime}$) since:\\
$\beta^{i_s} < \beta^{i^\prime}$
\fi


==> realtime_algo.tex <==
\section{Real Time Streaming Algorithm}

In this section, we will describe the algorithm for real time streaming assuming that we non-causally know the future bandwidth. We will further relax the assumption to consider prediction errors, and give an online algorithm. 

\subsection{Non-causal Algorithm}

The algorithm first finds the frames of base layer that can be fetched using a greedy algorithm. We start using the bandwidth to get all the base layers in order. In case we cannot obtain a frame by its deadline, it means that there is no way that till that point, I can get all the frames. Thus, we decide to skip the frame we could not fetch and start fetching the next frame. The policy continues, with an output of which frames could be fetched. More formally, this algorithm can be described as in Algorithm 1. We note that this algorithm tries to download as fast as possible. However, if a frame cannot be downloaded by its deadline, then that frame is skipped and the next frame is considered. If enough frames have been downloaded that miss the buffer capacity, the amount of download for the future chunks is reduced so that the buffer size is not violated. In each while loop, one of $i$ or $t$ is incremented and thus the best case and worst case complexity for this algorithm is $O(T)$ and $O(T^2)$ respectively. 

\begin{algorithm}
\caption{Algorithm 1: Greedy policy for Base Layer Scheduling }\label{euclid}
\begin{algorithmic}[]
\State {\bf Inputs:} $B(j)  \gets$ available bandwidth at time $j$, $r$ is the size of the base layer, $d$ is the startup delay, maximum buffer $B_m$.
\State {\bf Initialization: } Current frame downloading $i=1$, amount of data downloaded for frame $i$ is $D=0$, Current time $t=1$, Index of download $I=\phi$.
\While{$i\le T-d$ and $t\le T$}
\If {$B(t)< r-D$}
\State $D=D+B(t)$, $t=t+1$
\ElsIf {$B(t)\ge r-D$}
\State $B(t) = B(t) - (r-D)$, % Frame i BW is available and is thus used.
\If{$i\le T-d$ and $(|I \cap \{t-D+1, \cdots, i\}|+1)r\le B_m$}
% Frame is counted.
\State $I = I \cup i$
\State $i=i+1$, $D=0$.
\ElsIf {$(|I \cap \{t-D+1, \cdots, i\}|+1)r\le B_m$}
\State $i=i+1$, $D=r$.
\Else
\State  $D = B_m - |I \cap \{t-D+1, \cdots, i\}|r$, $t=t+1$.
\EndIf
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}




\begin{theorem} Among any class of algorithms, the above greedy algorithm provides the maximum number of base layer frames.
\end{theorem}
\begin{proof}
The proof follows by the greedy nature of the algorithm. At the time, the first frame is skipped implies that there is no bandwidth available to obtain all the frames till that time. Thus, one frame at least has to be skipped. We can extend the arguments to see that there is no strategy that can obtain less number of skipped frames.
\end{proof}

Having determined the frames that can be obtained for the base layer, we now form an optimization for obtaining the chunks at the higher layers. In order to do that, we assume that the base layer is downloaded for set $I_0$ of frames, and enhancement layer $i$ is downloaded for $I_i \subseteq I_{i-1}$ frames, $i = 1, \cdots, L$. With this, we wish to determine the amount of data that can be downloaded for the enhancement layer $I+1$. Let $xb(i,t)$ be the amount of data for base layer for frame $i$ downloaded in time $t$, and similarly $xe_j(i,t)$ represents the amount of data for enhancement layer $j$ for frame $i$ downloaded in time $t$. Then, we try to fill in gaps to download frames in enhancement layer $L+1$ given the decision for the earlier frames has already been made. 

\begin{equation}
maximize \sum_{i=1}^{T-d}\sum_{j=1}^{i+d} \gamma^{i} xe_{L+1}(i,j)
\end{equation}
$subject \  to$\\
\begin{equation}
\sum_{i=1}^{t-d}\sum_{j=1}^{t} xb(i,j) \geq r |I_0 \cap \{1, \cdots, t-d\}| \   \forall t=1,\cdots,T
\end{equation}
\begin{equation}
\sum_{i=1}^{t-d}\sum_{j=1}^{t} xe_q(i,j) \geq r_q|I_q \cap \{1, \cdots, t-d\}| \   \forall t=1,\cdots,T \   and \   q=1,\cdots, L
\end{equation}
\begin{equation}
 \sum_{j=1}^{i+d} xb(i,j) \leq r \forall i = 1, \cdots, T-d
 \end{equation}
\begin{equation}
 \sum_{j=1}^{i+d} xe_{q}(i,j) \leq r_q\  \forall i = 1, \cdots, T-d, q=1,\cdots, L+1
 \end{equation}
\begin{equation}
 \sum_{i=1}^{T-d} xb(i,j) +  \sum_{q=1}^{L+1}\sum_{i=1}^{T-d} xe_{q}(i,j)  \leq B(j) \  \   \forall j=1, \cdots, T, 
 \end{equation}
\begin{equation}
\sum_{i=t-d+1}^{T-d}\sum_{j=1}^{T} (xb(i,j)+\sum_{q=1}^{L+1}xe_{q}(i,j)) \leq M \   \forall t=1, \cdots, T 
\end{equation}
\begin{equation}
xb(i,j)=0\  \forall i \in I_0
\end{equation}
\begin{equation}
xe_{q}(i,j)=0\  \forall i \in I_{q},  q=1,\cdots, L
\end{equation}
\begin{equation}
xe_{L+1}(i,j)=0\  \forall i \in I_L
\end{equation}
\begin{equation}
xb(i,j) \geq 0
\end{equation}
\begin{equation}
xe_{q}(i,j) \geq 0\  \forall q=1,\cdots, I+1
\end{equation}

We note that $\gamma>1$ gives priority to later frames, and helps in getting most frames completely - since we did not explicitly include the integer constraint that the frames are either fully downloaded or not. The constraints here are all the properties the downloaded chunks at different levels have to satisfy. The first two constraints represent that the chunks of base and lower enhancement layers are downloaded in the sets decided. The next two constraints determine that the amount of data downloaded for a frame is no more than its size. The next two constraints are the bandwidth and buffer constraints. The next three constraints represent that no frame outside the set decided for the lower chunk is downloaded and further for the current enhancement layer decision, frame is not obtained unless the previous layer was downloaded. The last two constraints are the non-negativity constraints on the variables. 

This is a linear optimization, which can be solved easily. The approach is to fill in the gaps in the schedule to allow for the higher layer download. The frames which can be downloaded form the set $I_{I+1}$ for determining the next level. As a result of this Algorithm, we obtain the frames that can be obtained in each layer. We also take the partial frames for the highest layer since the partial frame for the highest layer can still be played. After the decision of quality of each frame is decided, they are obtained in sequence.






 \subsection{Real Time Scheduling with Prediction Error}
 
 In the presence of certain prediction error (assuming that the the error has zero mean), we use the schedule as decided above and start fetching the frames. However, if a frame is not completed by the deadline, the rest of the frame is not downloaded since there is no point of downloading content after its deadline. 
 
 There are a few adjustments we also make to the schedule. The first is random dropping. At each time, we drop the quality of frames by one enhancement layer whose deadline are within a threshold $\tau$, with probability proportional to the distance to deadline. This will help us in the case bandwidth is consistently lower in a certain regime that we are running very close to the run time, where we will reduce quality of chunks probabilistically. The second adjustment is random increase. In this approach, if we see that if the downloaded amount is more than the sum of predicted throughput by a threshold, we increase quality of the later chunks with probability proportional to the time left to download the chunk, and inversely proportional to the inverse of the quality of future chunks.
 

 \subsection{Real Time Online Scheduling Algorithm}

We assume that the optimization is performed very $\alpha$ time-instants and the prediction for a window of length $W$ is known. We first assume that the bandwidth is known perfectly. Assuming the bandwidth for the next $W$ time-instants, the proposed optimization framework is performed for all the frames that have not been downloaded so far and are within the first $W-d$ time instants of this window. If these frames are downloaded earlier, the rest of the frames are downloaded in the highest quality.

In the presence of prediction error, similar modifications are made as in the previous subsection. More precisely, the part of the frame not downloaded by its deadline is skipped. The random drop and random increase policies are also utilized for the schedule till the $W-d$ frames.




 %In some real scenarios we might be able to predict the bandwidth for sometime but we do not know what the bandwidth is going to be after a certain amount of time. Moreover, we want to deliver the video frames in the highest possible quality, but we do not want to make the decision that we take for current predicted window of time affecting the video quality of later frames. Therefore, online algorithm is more realistic in this case. OptBLSchedule algorithm and optimization formulation of previous sections can be used to find the optimum policy of fetching frames corresponding to the current $W$ seconds period. The optimum policy is recalculated every $\alpha$ seconds where $\alpha \leq W$. Practically  $\alpha \leq W/2$. Choosing $\alpha << W$ gives the best possible fetching policy. Every $k*\alpha$, the fetching policy is recalculated and the decision that was made for the fetching quality of the frames corresponding to the overlapping zone between the current and previous windows (frames from $k*\alpha+1$ to $(k-1)*\alpha+W$) could be changed in the recalculation point  $k*\alpha$. Fig. \ref{fig:onlineAlgo}  shows how online algorithm works. As we can see from the figure; for first period (P1), predicted bandwidth of a window of length W seconds is used to decide the fetching quality of frames that are corresponding to it, and after $\alpha$ seconds, the same calculation is done for the $2^{nd}$ period(P2). Moreover, the figure shows the overlapping zone, where frames corresponding to this zone are reconsidered in the 2nd window calculation and decisions of fetching their remaining  non-fetched part could be changed. However, these frames could be partially downloaded before time $\alpha$, so whatever belong to these frames, and it is downloaded before time $\alpha$ is already fetched and the re-calculation would consider the remaining non-fetched portion of them only. For example, If the bandwidth changed from high to low between W1 and W2, and the quality of frames that correspond to  $k*\alpha+1$ to $(k-1)*\alpha+W$ was decided to be in highest enhancement layer while current prediction shows that some frames corresponding to the current window (W2) might not be delivered completely before their deadline if those frames delivered in highest quality, then the decision that was made of fetching $k*\alpha+1$ to $(k-1)*\alpha+W$ in highest quality would change and priority would be given to fetching base layer of current frames to avoid any stalls. How often stalls can be avoided is function of $W$, $\alpha$ and of course the bandwidth profile itself. Having $W$ as large as possible and recalculation point $\alpha << W$ leads to better policy, Fig. \ref{fig:wAlpha} (b) shows how for fixed $\alpha$having higher prediction window size for the same bandwidth profile ($avgBw=1.6$) reduces the number of stalls. As we see from the figure for $\alpha=10$ when $W=40$. 11 frames out of 600 frames were not delivered. Having the window size $W=50$ reduces the number of stalls to $5$, and at $W=60$ we see that all frames were delivered completely. However, looking to Fig. \ref{fig:wAlpha} (a) for fixed window size ($W=120$) and average bandwidth ($avgBw=1.2$), having $\alpha=10$ leads to deliver all frames, and as $\alpha$ increases we start see more stalls and the reason is obviously more frames delivered in high quality for current window and not being considered for next window means the algorithm is more optimistic in delivering current frames while less conservative about the future. After enhancing for fetching frames that correspond to the current predicted window, algorithm 3 is used to fetch the base layer of later frames if there is still available bandwidth.
 \begin{figure*}
\centering
\epsfig{file=online_algo.pdf, height=3in, width=5in}
\caption{Online algorithm}
\label{fig:onlineAlgo}
\end{figure*}
 \begin{figure*}
 \centering
\epsfig{file=figures/w_alpha_stalls.eps, height=2in, width=3in}
\epsfig{file=figures/alpha.eps, height=2in, width=3in}
\caption{(a)Number of stalls vs window size , and (b) Number of stalls vs $\alpha$}
\label{fig:wAlpha}
\end{figure*} 

==> realtime_sims.tex <==
\section{Real time algorithm\\ simulation and results}
    To evaluate the algorithm, we first created an example scenario where we assumed that a user is moving on a road and a tunnel is ahead of him. The user is downloading a 3 minute video. The moving scenario and the real bandwidth are shown in Fig. \ref{fig:tunnelEx}. As seen from the figure the user experience 3 zones with average bandwidth of about 1.8Mbps. We considered the base layer and $3$ enhancement layers with start up delay of $6$ seconds. We compared our algorithm with $3$ naive strategies. Naive1 which works as follow; It fetches the base layer of all frames before it starts to fetch the $1st$ enhancement layer of frames that can have their $1st$ enhancement layers before their deadline. Once it fetches the $1st$ enhancement layer, it moves to fetching the $2nd$ enhancement layer and so on. Naive 2, and naive3 fetch all layers of frame $i$ before start fetching all layers of frame $j$ when $i < j$.
      \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
 Algo &  \#stalls & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR\\ \hline
 naive1 &  0 & 117 & 13 & 4 & 41 & 1.375\\
 naive2 & 40 & 0 & 0 & 0 & 135 & 1.645\\
 naive3 & 29 & 31 & 0 & 0 & 115 & 1.59 \\
 SVC & 0 &  8 & 107 &  0 & 60 & 1.76\\ \hline\end{tabular}
 \caption{Tunnel scenario results}
 \label{tab:tunnel}
\end{table}
    \begin{figure}
\centering
\epsfig{file=figures/playRate_25_05_25_pe_0_180s.eps, height=2in, width=3in}
%\epsfig{file=toy_bw_results/cdf_25_05_25_pe_0_180s.pdf, height=3in, width=3in}
\caption{Playback rate of the tunnel scenario}
\label{fig:tunnel}
\end{figure}
 It is clearly shown from table \ref{tab:tunnel} and play back Fig. \ref{fig:tunnel}, both naive 2 and 3 are running in many stalls with 40 stalls for naive 2 and 29 stalls for naive 3. The reason behind that is the very optimistic behavior of both algorithms in delivering current frames in highest possible enhancement layer without considering the future. Delivering current frame in highest enhancement layer may lead to loosing enough bandwidth to deliver some of next frames even in base layer. What happened is that, initially ($1^{st}$ minute), the available bandwidth was high and add to that a start up delay of $6s$, so naive 2 and naive 3 went to fetch all frames corresponding to the 1st minute in highest enhancement layer ($3^{rd}$ enhancement layer)) . Naive 2 and 3 work on a way where if there is an available bandwidth at any time instant, they go to get $3^{rd}$ enhancement layer for frame $i$ before the base layer of frame $j$ where $i < j$. However, according to the average bandwidth of 1.8, where in average frames can be delivered in $2^{nd}$ enhancement layer, if a frame is delivered in $3^{rd}$ enhancement layer there will be high possibility that another one will not be delivered at all. And actually this is exactly what happened according to the given scenario. After the user entered the tunnel, we start to see naive 2 and naive 3 running into stalls, and most of the frames which their fetching time is corresponding to the time spent under the tunnel were not delivered. In contrast to that, naive 1 is very conservative to the point that many frames are delivered in low quality even though the bandwidth allows for higher quality to be delivered. Naive 1 does not run into stalls, but it delivers frames in the lowest average quality of $1.375Mbps$. It does not start fetching $1^{st}$ enhancement layer of remaining frames until it fetches the base layer of all frames. It does the same thing when it moves to fetching $2^{nd}$ enhancement layer if the bandwidth allows to do so. As we see from figure(), naive 1 played back the 1st 120s (2/3 of the video) in the base layer quality even though the average bandwidth would allow for higher paly back quality. SVC is less conservative than naive 1 and less optimistic than naive 2 and 3. It works in between, where It delivers the frames in the best possible quality considering avoiding future stalls. It optimizes over which frame should be delivered in what quality considering the whole bandwidth profile and all frames. As the table shows, SVC has the highest average of $1.76$ which reflects best utilization of the bandwidth with $0$ stalls. Even the bandwidth is high in the beginning, SVC does not go to fetch the frames in highest quality level, instead it smooths the quality over all frames. figure() shows that even after a minute the user is under the tunnel, but the playback quality of SVC is still stable, and the user is still  watching the frames in the $1^{st}$ enhancement layer quality. Moreover, the quality jumped to the $3^{rd}$ enhancement layer when the user left the tunnel.
  We notice that naive 2 and 3 do not deliver about  $23\%$ and $18\%$ of the frames, and naive 1 delivers about $68\%$ of the frames in the base layer quality. However, SVC delivers more than $95\%$ of the frames in a quality $\geq$ $1^{st}$ enhancement layer.
Let's take more realistic scenario where the bandwidth is predicted with a prediction error of $20\%$, so we can see how prediction error can affect the results. To do so, we simulate a video using the real and predicted bandwidth profiles which are shown in Fig. \ref{fig:tunnelPe}. We again compared the performance of our algorithm with naives 1, 2, and 3.

 \begin{figure}
\centering
\epsfig{file=figures/rpB.eps, height=2in, width=3in }
\caption{Real and predicted bandwidth for the tunnel scenario}
\label{fig:tunnelPe}
\end{figure}
 We see from the results on table \ref{tab:tunnelPeR} and the figure \ref{fig:tunnelPeR} ,  that even with $20\%$ prediction error SVC is still fetching the frames in highest quality on average with value of 1.755. In the online case, algorithm x with RED which were described in section () are used to help making the decision of what to be fetched at any time slot if the real bandwidth is different from the predicted one. According to the predicted bandwidth, certain policy is pre-decided. However, on every time slot algorithm x with RED modify the decision if the real bandwidth is not equal to the predicted one by deferring fetching frames in case $BR(i) < BP(i)$ with random probability of quality drop, and fetching as much as BR(i) allows of later frames if $BR(i) \geq BP(i)$. Therefore, in real scenarios, delivered quality might be less than the pre-decided one because of prediction error. For example, looking into figure(), we see drop on the quality of the frames $140$, and $142$. According to the predicted bandwidth a decision was made to deliver all frames beyond $115th$ frame in highest enhancement layer quality. However, because of the teal bandwidth was less than the predicted one and there was no enough bandwidth to fetch frames $140$, and $142$ in the pre-decided quality before their deadlines, the decision is changed and both frames where fetched in $2^{nd}$ enhancement layer quality.
 \\
     \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
 Algo &  \#stalls & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR\\  \hline
 naive1 &  0 & 115 & 12 & 5 & 43 & 1.388\\
 naive2 & 33 & 5 & 0 & 0 & 137 & 1.70\\
 naive3 & 24 & 20 & 4 & 6 & 121 & 1.697\\
 $SVC$ & 0 &  8 & 107 &  2 & 58 & 1.7553\\ \hline\end{tabular}
  \label{tab:tunnelPeR}
   \caption{Tunnel scenario with 20\% prediction error results}
\end{table}
 \begin{figure}
\centering
\epsfig{file=figures/play_rate_svc_W_180_alpha_30_sf_1_z_180_5_startup_delay_20_percent_prediction_error_vs_naive.eps, height=2in, width=3in}
%\epsfig{file=toy_bw_results/quality_svc_W_180_alpha_30_sf_1_z_180_20_percent_prediction_error_vs_naive.pdf, height=1.8in, width=2in}
\caption{Playback rate of the tunnel scenario with 20\% prediction error}
\label{fig:tunnelPeR}
\end{figure}
Real tunnel like scenario:\\
 For this section we collected real trace where a hypothesis of tunnel like is already exist and we compared our algorithm's performance with all of the 3 naive strategies. We assumed $20\%$ of prediction error where the real and predicted bandwidths are shown in Fig. \ref{fig:realTunnelBw}. According to the figure, we see 3 zones, 2 zones with fairly good average bandwidth and a zone in between where the bandwidth is running low (tunnel like scenario). Table \ref{tab:realTunnelPeR} shows how SVC was able to deliver frames in highest average quality (1.69) without running into stalls. Naive 2 and 3 come second in term of high average (1.47, and 1.47)), but both of them are running into stalls with 24 stalls each. Naive 1 does not run into stalls, but it delivers the frames in the lowest quality in average (1.37). From figure \ref{fig:realTunnelPeR}, we see that because naive 2 and 3 do not account for the future, They deliver first few frames  at the highest quality level, but  the cost is that most of the frames that corresponding to the through time are not delivered. Naive 2 and 3 do not deliver almost $20\%$ of the frames.  In contrast to that, naive 1 is very conservative to the point that it starts fetching frames in $1st$ enhancement layer very late on time (after about 1 minutes). Moreover, it delivers about $60\%$ of the frames in the base layer. SVC works in between, it jumps to $1st$ enhancement layer very early in time (from $1st$ frame). It does not go as high as naive 2 and 3 do because it accounts for later frames, and it is not as too conservative as naive 1 does. It optimizes over the highest quality needed for delivering the current frame without hurting later frames.\\
 \begin{figure}
\centering
\epsfig{file=figures/bp_br_tunnel_real.eps,height=2in, width=3in}
\label{fig:realTunnelBw}
 \caption{Real tunnel like bandwidth profile}
\end{figure}
  \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
 Algo &  \#stalls & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR\\ \hline
 naive1 &  0 & 76 & 10 & 5 & 24 & 1.37 \\
 naive2 & 24 & 20 & 3 & 7 & 61 & 1.47\\
 naive3 & 24 & 19 & 5 & 8 & 59 & 1.47 \\
 $SVC$ & 0 &  1 & 84 &  19 & 11 & 1.69\\ \hline\end{tabular}
  \label{tab:realTunnelPeR}
   \caption{Real tunnel like scenario with 20\% prediction error results}
\end{table}
 \begin{figure}
\centering
\epsfig{file=figures/playRate_real_tunnel_df13_120s.eps, height=2in, width=3in}
%\epsfig{file=toy_bw_results/cdf_real_tunnel_df13_120s.pdf, height=2in, width=3in}
\caption{Playback rate for real tunnel like scenario with 20\% prediction error}
\label{fig:realTunnelPeR}
\end{figure}
Now we want to consider a scenario where the bandwidth is oscillating between as high as it is enough to deliver frames in highest quality (Ex. 2.5Mbps) and as low as it can not allow for fetching frames even in base layer quality (Ex. 0.5Mbps) which is actually a practical scenario with mobile users. To explain how SVC does with compare to naive strategies we used the bandwidth profile that is shown in Fig. \ref{fig:oscil} with average bandwidth of $1.5$, and we assumed a video of 2 minutes length.\\
 \begin{figure}
\centering
\epsfig{file=figures/bw_cos_f_60_120s.eps, height=2in, width=3in}
\caption{Oscillation bandwidth profile}
\label{fig:oscil}
\end{figure}
 because of the oscillation, it is expected that naive 2 and 3 would run into many stalls. And that is exactly what table     \ref{tab:oscilR} and Fig. \ref{fig:oscilR} shows. naive 2 do not completely deliver 37 frames, and naive 3 do not completely deliver 36 frames. The reason behind that is agai the same, both naive 2 and 3 go to fetch frames in highest quality level whenever it is possible (around 2.5Mbps region), and when the bandwidth runs low (around 0.5 Mbps) they do not find enough bandwidth to deliver frames even in base layer. Even though they deliver about $50\%$ of frames in a quality that is in the $1st$ enhancement layer and higher, they fail to deliver $30\%$ of the frames. Naive 1 is able to deliver all frames, but more than 70 seconds out of 120s video length is played back in base layer, and about $60\%$ of the frames are delivered in the base layer quality . However, SVC does the best job among all strategies where It delivers frames in highest average quality ($1.544$Mbps). Even it does not jump immediately to fetch frames in enhancement layers, it does not wait for long time as naive 1 does. As shown in Fig. \ref{fig:oscilR}, after about 20 seconds from the start, and exactly where the bandwidth is very low, SVC starts playing back frames in $1st$ enhancement layer quality, That is because the enhancement layer corresponding to this time frames were fetched early on. About $80\%$ of the frames are delivered in the $1st$ enhancement layer quality or more.\\
  \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
 Algorithm &  \#stalls & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR\\ \hline
 naive1 &  0 & 71 & 28 & 3 & 13 & 1.338\\
 naive2 & 37 & 13 & 5 & 6 & 54 & 1.289\\
 naive3 & 36 & 13 & 8 & 9 & 49 & 1.286 \\
 $SVC$ & 0 &  24 & 77 &  4 & 10 & 1.544\\
  \hline\end{tabular}
    \label{tab:oscilR}
     \caption{Oscillation scenario results}
\end{table}
  \begin{figure}
\centering
\epsfig{file=figures/playRate_cos_f_60_120s.eps, height=2in, width=3in}
%\epsfig{file=toy_bw_results/cdf_real_tunnel_df13_120s.eps, height=2in, width=3in}
\caption{PlayBack rate for oscillation scenario}
 \label{fig:oscilR}
\end{figure}
   Last example was short video assuming full knowledge of the bandwidth with no prediction error. However, to make the scenario close to the reality, let's assume the same oscillating bandwidth profile but for a video of $10 minutes$ length and the bandwidth profile shown in Fig \ref{fig:oscilPe}. Moreover, we use the online version where the bandwidth can be predicted for a window of $W$ seconds. Let us assume that  $W=2 minutes$ minutes, and fetching policy recalculation every $30s$ ,$\alpha=30s$. We assume prediction error (PE) and the prediction error is increasing as time gets far from the re-calculation point $k\alpha$. Finally, we assume that the prediction error of the $1st$ 20 seconds starting at $k\alpha+1$ to $k\alpha+20$ is $10\%$, and the prediction error of the next 20 seconds is $15\%$ and so on. i.e PE=[10 15 20 25 30 35].
    \begin{figure}
\centering
\epsfig{file=figures/bw_cos_600s_pe_v.eps, height=2in, width=3in}
\caption{Long video, oscillating bandwidth profile scenario with prediction error}
\label{fig:oscilPe}
\end{figure}
  Table \ref{tab:oscilPeR} shows a compares the SVC, $W=120$, and $\alpha=30$, $SVC\_30$, with the 3 naive strategies. We see from table \ref{tab:oscilPeR} and the play back Fig.\ref{fig:oscilPeR} that even though the SVC does not have a prediction of the full video duration bandwidth up front, it still have the best average play rate (1.468 Mbps), and it does not run into stalls. To reduce the effect of early decisions on later frames $\alpha$ has practically chosen to be much less than the window size $W$, so every $k*\alpha$, the fetching policy is recalculated and the decision that was made for fetching frames from $k*\alpha+1$ to $(k-1)*\alpha+W$ could be changed at the recalculation point  $k*\alpha$. We see from the play rate and the CDF figures that SVC delivers about $75\%$ of the frames in $1st$ enhancement layer. It is expected that the performance of the online algorithm could be lower than the offline version, but we still see better performance than the naive strategies in the oscillating scenario. from Fig.\ref{fig:oscilPeR}, we see that naive 2 and 3 run into many stalls, They do not deliver about $30\%$ of the frames. Naive 1 fetches most of the frames in the base layer and by the time the video reaches about 420second of 600seconds video which is about $70\%$ of the video time, quality changes to $1st$  enhancement layer which means that $70\%$ of the frames are delivered in the base layer and by the time naive 1 jumps to fetch higher layer, the video is reaching its end.
 \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
 Algorithm &  \#stalls & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR\\ \hline
 naive1 &  0 & 414 & 64 & 19 & 98 & 1.325 \\
 naive2 & 179 & 102 & 24 & 20 & 270 & 1.278\\
 naive3 & 177 & 104 & 25 & 26 & 263 & 1.278 \\
 $SVC$ & 0 &  159 & 418 &  13 & 5 & 1.468\\
  \hline\end{tabular}
  \label{tab:oscilPeR}
  \caption{Long video, oscillating scenario results}
\end{table}
\begin{figure}
\centering
\epsfig{file=figures/playRate_cos_f_60_600s_pe_v.eps, height=2in, width=3in}
%\epsfig{file=toy_bw_results/cdf_cos_f_60_120s.pdf, height=1.8in, width=2in}
\caption{PlayBack rate for long video oscillating scenario}
\label{fig:oscilPeR}
\end{figure}

 In reality, scenarios might not be exactly any of the above mentioned. Therefore, in next section we will show comparisons of SVC with other naive strategies for real collected bandwidth profiles. We will see that even running online algorithm with prediction error SVC still outperform all naive strategies in many scenarios; Especially, when in average the bandwidth can allow frames to be fetched in $1st$ enhancement layer (moderate bandwidth regime).\\

  \section{Real scenario simulation}
 We start with short videos and offline algorithm (full non causal knowledge of the bandwidth profile)\\
\subsection{offline algorithm}
We simulated a video of $2$ minute length with 4 average bandwidth level for real collected bandwidth traces defined as very good regime with average bandwidth ($Avg BW=2.5$), good regime ($Avg BW=1.80$) , moderate regime ($Avg BW=1.52$), and bad regime ($Avg BW=1.1$). We used 2 bandwidth profiles. In first profile, in average, bandwidth starts at good regime and decreases with time, and the other profile is the flip of the $1st$ one. Both bandwidth profiles are shown in Fig.  \ref{fig:bwProfiles} (a) and (b) \\
 \begin{figure*}
\centering
\epsfig{file=figures/bw_1.eps, height=2in, width=3in}
\epsfig{file=figures/bw_2.eps, height=2in, width=3in}
\caption{Real Bandwidth Profiles}
 \label{fig:bwProfiles}
\end{figure*}
\subsubsection{Bandwidth profile 1}
In the very good regime (Avg BW=2.5Mbps), and as table \ref{tab:offlineReal} and Fig. \ref{fig:offlineResults} (a) show, our algorithm does as good as the algorithm that fetches the higher layers of the current frame before fetching the base layer of the next frame. We see that even in good regime (Avg BW=1.8Mbps) these algorithms run into stalls while our algorithm keeps balancing between moving to higher layers and avoiding stalls. Because in the very good regime the average bandwidth is high, all algorithms deliver all frames before their deadlines and there are no stalls in any of them. However, the average delivered quality of SVC and naive 2 are the highest with value of 2.133. Both SVC and naive 2 deliver all $115$ frames at the $3^{rd}$ enhancement layer quality (the highest), and as expected the average quality of naive 1 is the lowest with a value of 1.834 which means that the average delivered quality is the $2^{nd}$ enhancement layer. Naive 1 delivers  about $50\%$ of the frames in a quality that is $\leq 2^{nd}$ enhancement layer.  As we previously mentioned, naive 1 does not start fetching $1^{st}$ enhancement layer until it fetches the base layer of all frames, and by the time it fetches base layer of all frames, many frames have already been played back in base layer quality, so their $1^{st}$ enhancement layer wont be fetched, instead the algorithm will start fetching the $1^{st}$ enhancement layer of the frames that are not played back yet. In good regime (Avg BW=1.8Mbps) When on average frames can be delivered in $2^{nd}$ enhancement layer, we start seeing naive 2 and 3 running in stalls because they are very optimistic in delivering frames in higher enhancement layer. Delivering current frame in highest enhancement layer may lead to loosing enough bandwidth to deliver the next frame even in base layer. What happen to naive 2 and 3 is that if there is an available bandwidth at any time instant, they give priority to fetching the $3^{rd}$ enhancement layer for frame $i$ before the base layer of frame $j$ when $i < j$, and according to the average bandwidth of 1.8, in average the frames can be delivered in the $2^{nd}$ enhancement layer; Therefore, if a frame is delivered in $3^{rd}$ enhancement layer there will be high possibility that another one would not be delivered at all. In contrast to that, naive 1 is very conservative to the point that many frames are delivered in low quality even though the bandwidth allows for higher quality to be delivered. SVC is less conservative than naive 1 and less optimistic than naive 2 and 3. It works in between and in average it delivers the frames in the best possible quality considering avoiding stalls. It optimizes over which frame should be delivered in which quality considering the whole bandwidth profile and all frames. As the table \ref{tab:offlineReal} and Fig. \ref{fig:offlineResults} (b) shows, In good regime, SVC has the highest average $1.883$ with $0$ stalls. Moreover 108 out of $120$ frames are delivered in $2^{nd}$ enhancement layer. naive 1 does not run into stalls but it has the lowest average quality $1.597$. naive 2 and naive 3 have average quality better then naive 1. However, they do not meet deadline of some frames. For naive 1, we can see that more than $50\%$ of the frames are delivered in quality $\leq 1^{st}$ enhancement layer. Naive 2 and 3 delivers about $50\%$ of frames in quality of highest enhancement layer, but they run into stalls and very high variability in the playback quality.
When in average frames can be delivered in $1^{st}$ enhancement layer (Avg BW=2.5Mbps), as table \ref{tab:offlineReal} and Fig. \ref{fig:offlineResults} (c) shows, SVC delivers frames in highest average of $1.593$. Moreover, SVC does not run into stalls. naive 2 and 3 do not violate the deadline of about $27\%$ and $21\%$ of the frames respectively. naive 1 has no stalls but low quality per frame with compare to SVC. SVC delivers more than $90\%$ of the frames in quality of $1^{st}$ enhancement layer while naive 1 delivers more than $50\%$ of the frames on the base layer quality. Naive 2 and 3 deliver some frames on the highest quality level but the cost is not delivering some other frames.
In conclusion, offline SVC can do as good as the optimistic algorithms in the high bandwidth regime because of its prior knowledge of the full bandwidth and the optimization over what to fetch at what time. It does nice job in good regime as well since it balances between between being so optimistic and so conservative. the power of the introduced algorithm can be seen  in the regime where very optimistic algorithm run in many stalls and very conservative algorithm do not fully utilize the available bandwidth.\\
 \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Avg\_BW & Algo & \#s & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR \\ \hline
 2.5Mbps & naive1 &  0 & 16 & 23 & 19 & 57 & 1.834  \\
                   &naive2 & 0 & 0 & 0 & 0 & 115 & 2.133  \\
                   &naive3 & 0 & 0 & 0 & 5 & 110 & 2.12  \\
                   &SVC & 0 &  0 & 0 &  0 & 115 & 2.133 \\ \hline \hline
  1.8Mbps &naive1 &  0 & 35 & 42 & 7 & 31 & 1.597 \\
 		&naive2 & 14 & 8 & 4 & 1 & 88 & 1.778 \\
 		&naive3 & 7 & 15 & 11 & 18 & 64 & 1.77  \\
 		&SVC & 0 &  0 & 0 &  108 & 7 & 1.883 \\ \hline \hline
  1.5Mbps & naive1 &  0 & 60 & 26 & 3 & 26 & 1.449 \\
                   &naive2 & 33 & 13 & 5 & 0 & 64 & 1.377 \\
                   &naive3 & 26 & 22 & 13 & 9 & 45 & 1.365\\
                  &SVC & 0 &  2 & 112 &  1 & 0 & 1.593\\ \hline \hline
  1.25Mbps &naive1 &  0 & 86 & 11 & 6 & 12 & 1.27\\
 		&naive2 & 55 & 12 & 2 & 0 & 46 & 0.99\\
  		&naive3 & 50 & 20 & 8 & 4 & 33 & 0.97\\
 		&SVC & 0 &  66 & 49 &  0 & 0 & 1.294\\ \hline \hline\end{tabular}
		  \label{tab:offlineReal}
		   \caption{Offline algorithm results for Bandwidth Profile 1}
\end{table}
 %\includegraphics[scale=0.45]{offline_cdfs/bw248}
 \begin{figure*}
\centering
\epsfig{file=figures/play_rate_svc_W_120_alpha_10_sf_4_z_120_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/play_rate_svc_W_120_alpha_10_sf_55_z_120_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/play_rate_svc_W_120_alpha_10_sf_65_z_120_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/play_rate124.eps, height=2in, width=3in}
\caption{PlayBack rate , offline, Bandwdith Profile 1}
 \label{fig:offlineResults}
\end{figure*}

\subsubsection{Bandwidth profile 2}
In the case of bandwidth profile 2 which is shown in Fig. \ref{fig:bwProfiles}  (b) , the low bandwidth regime comes first and as the time goes the bandwidth improves in average.
As shown in table \ref{tab:offlineRealBw2} and Fig. \ref{fig:offlineResultsBw2} (a),  In high average bandwidth (2.5Mbps),SVC and naive 1 do not run into stalls. However, SVC has the highest average quality with $1.91$ and most of frames are delivered in $2^{nd}$ enhancement layer. It is clearly shown that even the average bandwidth is high, naive 2 and naive 3 run into stalls because of the low bandwidth in the beginning. For SVC, we see that 80 out of 115 frames are delivered in $2^{nd}$ enhancement layer, and 27 are delivered in highest quality level. Naive 1 delivers $50\%$ of the frames in the quality of the base layer. naive 2 and naive 3 deliver 86 and 74 frames out of 115 frames in highest quality level but on the cost of not delivering some other frames. In the case of average Bw of $1.825 Mb/s$, we can see from the table \ref{tab:offlineRealBw2} and Fig. \ref{fig:offlineResultsBw2} (b) that because the low bandwidth comes first even the average bandwidth is as high as 1.825 Mb/s, naive 2 and naive 3 do not deliver more than $25\%$ of the frames. Naive 1 delivers all frames on average quality of $1.28$ and more than $75\%$ of the frames are delivered on quality of the base layer. However, SVC has the highest average quality of delivery with value of $1.523$, and more than $60\%$ of the frames are delivered on quality that is $\geq 1^{st}$ enhancement layer. In the case of average Bw of $1.544 Mb/s$, naive 2 and naive 3 do not deliver about $40\%$ of the frames. naive 1 deliver all frames on average quality of $1.24$ and more than $80\%$ of the frames are delivered on quality of the base layer. However, SVC has the highest average quality of delivery with value of $1.359$, and more than $30\%$ of the frames are delivered on quality that is $\geq 1^{st}$ enhancement layer. For the very low regime , Average Bw of $1.25 Mb/s$, all of the algorithms run into stalls. However SVC has the lowest number of stalls with 21 non delivered frames which is less than half of the number of stalls of naive 1 and about 1/3 of naive 2 and naive 3. SVC deliver frames in highest average quality with value of $1.09$.
In conclusion, in this scenario naive 2 and 3 experience more stalls in the beginning even in the high average because of their optimistic behavior. However, in high average bandwidth scenario, SVC and naive 1 do not run into stalls, but in low average bandwidth scenario, naive 1 may keep fetching frames that would not meet their deadline requirements while SVC skip fetching those frames, so SVC reduces the number of the non delivered frames.

\begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Avg\_BW &Algo &  \#stalls & \#b &  \#e1 &  \#e2 &  \#e3 &  APBR\\ \hline
 2.5Mbps&naive1 &  0 & 59 & 23 & 5 & 28 & 1.467\\
 &naive2 & 11 & 7 & 4 & 7 & 86 & 1.829\\
 &naive3 & 8 & 11 & 8 & 14 & 74 & 1.813\\
 &SVC & 0 &  0 & 8 &  80 & 27 & 1.91\\ \hline \hline
 1.8Mbps&naive1 &  0 & 90 & 4 & 0 & 21 & 1.280\\
 &naive2 & 33 & 22 & 3 & 4 & 53 & 1.293\\
 &naive3 & 31 & 26 & 3 & 8 & 47 & 1.284\\
 &SVC & 0 &  43 & 45 &  1 & 26 & 1.523\\ \hline\hline
 1.5Mbps&naive1 &  0 & 95 & 2 & 1 & 17 & 1.240\\
 &naive2 & 46 & 19 & 4 & 6 & 40 & 1.071\\
 &naive3 & 44 & 23 & 5 & 7 & 36 & 1.064\\
 &SVC & 0 &  77 & 12 &  2 & 24 & 1.359\\ \hline\hline
 1.25Mbps&naive1 &  29 & 69 & 4 & 1 & 12 & 0.934\\
 &naive2 & 63 & 14 & 3 & 3 & 32 & 1.813\\
 &naive3 & 62 & 16 & 4 & 6 & 27 & 0.802\\
 &SVC & 12 &  77 & 2 &  1 & 23 & 1.185\\ \hline\end{tabular}
   \label{tab:offlineRealBw2}
    \caption{Offline algorithm results for Bandwidth Profile 2}
\end{table}
 \begin{figure*}
\centering
\epsfig{file=figures/bw2_play_rate25.eps, height=2in, width=3in}
\epsfig{file=figures/bw2_play_rate1825.eps, height=2in, width=3in}
\epsfig{file=figures/bw_2_play_rate_svc_W_120_alpha_10_sf_6_z_120_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/bw2_playRate_124.eps, height=2in, width=3in}
\caption{PlayBack rate , offline, Bandwdith Profile 2}
\label{fig:offlineResultsBw2}
\end{figure*}


 \subsection{Online algorithm}
 We start with evaluating the effect of $\alpha$ and the prediction error on the performance of our algorithm, and then we compare our algorithm with the 3 naive strategies.\\
 
 \textbf{Effetc of $\alpha$}:  The optimum policy is recalculated every $\alpha$ seconds where $\alpha \leq W$. Choosing $\alpha << W$ leads to better fetching policy. Every $k*\alpha$, the fetching policy is recalculated and the decision that was made for fetching quality of the frames corresponding to the overlapping zone between the current and previous windows (frames from $k*\alpha+1$ to $(k-1)*\alpha+W$) could be changed in the recalculation point  $k*\alpha$. To evaluate the effect of $\alpha$, we simulated online algorithm for downloading a video of 600 second length. We assumed a prediction window of size 2 minutes, $W=120$, and average bandwidth ($avgBw=1.2$). Moreover, we assume bandwidth profile 3 where bandwidth starts at higher values and decreases over time. having $\alpha=10$ leads to deliver all frames, and as $\alpha$ increases we start to see more stalls and the reason is obviously more frames delivered in high quality for current window and not being considered for next window means the algorithm is more optimistic in delivering current frames while less conservative about the future. After enhancing for fetching frames that correspond to the current predicted window, algorithm 3 is used to fetch the later frames in highest quality level if there is still available bandwidth.   \\
   \begin{figure}
 \centering
\epsfig{file=figures/alpha.eps, height=2in, width=3in}
\caption{Number of stalls vs $\alpha$}
\label{fig:wAlpha}
\end{figure} 

 \textbf{Effetc of Prediction Error}:  To evaluate the effect of the prediction error on the online algorithm, we simulated a video of 10 minute length. We assumed a prediction window of size 2 minutes, $W=120$, recalculation every 30 seconds ($\alpha=30$), and average bandwidth ($avgBw=1.2$). Moreover, we assume bandwidth profile 3 where bandwidth starts at higher values and decreases over time. We test the algorithm for prediction error of $10\%$, $20\%$, $30\%$, and $40\%$.\\
    


 
 To test the performance of our algorithm with compare to the 3 naive strategies, we simulated a video of $10$ minute length, using bandwidth profiles 3 and 4 which are shown in Fig. \ref{fig:bwProfiles34}. We assume that we have bandwidth prediction of $2$ minutes ahead, window size of $120$ seconds, and we chose $\alpha=20$ seconds. We considered prediction error (PE), and the prediction error is increasing as time gets far from the recalculation point $k\alpha$. we assume that the prediction error of the 1st 20 seconds starting at $k\alpha+1$ to $k\alpha+20$ is $10\%$, and the prediction error of the next 20 seconds is $15\%$ and so on. i.e PE=[10 15 20 25 30 35].\\
  \begin{figure}
\centering
\epsfig{file=figures/bp3.eps, height=2in, width=3in}
\epsfig{file=figures/bp4.eps, height=2in, width=3in}
\caption{Real Bandwidth Profiles 3 and 4}
 \label{fig:bwProfiles34}
\end{figure}

 \subsubsection{Bandwidth profile 3}
In the case of very good regime, Average Bw of $2.5 Mb/s$, as table \ref{tab:onlineReal} and Fig. \ref{fig:onlineResults} (a) shows, even though the low bandwidth comes later and even with prediction error specified above, our algorithm does as good as naive 2 and 3. Because the average bandwidth is high, all algorithms deliver all frames and there are no stalls in all of them. However, SVC and naive 2 have the highest average play rate. Both of them deliver the all the frames at the highest quality level. As expected the average quality of naive 1 is the lowest with a value of 1.79 which means that the average delivered quality is the $2^{rd}$ enhancement layer. 90\% of the fames using naive 1 are delivered in quality $Q \geq 1.067$. However $50\%$ is $\leq 1.867$ which means more than $50\%$ of the frames are delivered in quality that is $\leq 2^{nd}$ enhancement layer. In other hand,almost all frames on mostly SVC and naive 2, and naive 3) or are delivered on the highest enhancement layer ($3^{rd}$ enhancement layer). In the case of average Bw of $1.846 Mb/s$, as expected when the average bandwidth goes bellow the point of delivering all frames in highest quality level, we start to see naive 2 and naive 3 run into stalls. As the table and \ref{fig:onlineResults} (b)  show SVC has the highest average $1.854$ and $90\%$ of frames are delivered on a quality $\geq 1^{st}$ enhancement layer. naive 1 does not run into stalls but it has the lowest average quality $1.554$, and it delivers more than $50\%$ of the frames in quality $\leq 1^{st}$ enhancement layer. naive 2 and naive 3 have average quality better then naive 1. However, they do not deliver some frames. When the average Bw is equal to $1.562 Mb/s$ where in average frames can be delivered in $1^{st}$ enhancement layer we see as shown in table \ref{tab:onlineRealBw2} and Fig. \ref{fig:onlineResults} (c), SVC delivers frames in the highest average of $1.564$. Moreover, SVC does not run into stalls. Naive 2 and 3 do not deliver more than $25\%$ of the frames. naive 1 has no satlls but low quality per frame with compare to SVC. SVC delivers more than $50\%$ of the frames in quality $\geq$ $1^{st}$ enhancement layer while naive 1 delivers more than $50\%$ of the frames on the base layer quality. Naive 2 and 3 deliver some frames on the highest quality level but the cost is not delivering high percentage of the frames.
In the very low average bandwidth, average Bw of $1.248 Mb/s$, and specifically when the very low bandwidth comes later, the online SVC optimizes over current window and it does not have an idea that the bandwidth is going to run low for next few windows, so it would prioritize fetching higher enhancement layers of current frames over base layer of later frames, so when the bandwidth run low later, later frames might not be completely fetched in their window time.  Therefore, and as shown in table table \ref{tab:onlineReal} and Fig. \ref{fig:onlineResults} (d), SVC can not beat naive 1 in term of fetching all frames in this very low average bandwidth under this bandwidth profile scenario. However, if it is known upfront that the average bandwidth is very low, the greedy part of our algorithm can do better than naive 1 in term of avoiding stalls. Intuitively, OptBLSchedul algorithm uses predictability to skip frames that would not meet their deadline requirements, so the number of non fetched frames will be minimized. It is clearly shown from table table \ref{tab:onlineRealBw2} and Fig. \ref{fig:onlineResults} that naive 1 deliver frames in  the highest average quality with value of 1.25, and it does not run into stalls. Naive 2 and 3 do not deliver more than $50\%$ of the frames. online SVC with $W=120$ and $\alpha=20$ does not completely deliver about $18\%$ of the frames.

\begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Avg\_BW&Algo&\#stalls& \#b&\#e1&\#e2 &\#e3 &APBR\\ \hline
 2.5Mbps&naive1 &  0 & 106 & 133 & 81 & 275 & 1.79\\
 &naive2 & 0 & 0 & 0 & 0 & 595 & 2.133\\
 &naive3 & 0 & 6 & 7 & 27 & 555 & 2.12\\
 &SVC & 0 &  0 & 0 &  0 & 595 & 2.133\\ \hline\hline
 1.8Mbps&naive1 &  0 & 220 & 187 & 38 & 150 & 1.554\\
 &naive2 & 84 & 36 & 11 & 4 & 460 & 1.755 \\
 &naive3 & 45 & 73 & 70 & 73 & 334 & 1.745\\
 &SVC & 0 &  41 & 220 &  18 & 316 & 1.854\\ \hline\hline
 1.5Mbps&naive1 &  0 & 330 & 124 & 20 & 121 & 1.421\\
 &naive2 & 186 & 64 & 11 & 6 & 328 & 1.339\\
 &naive3 & 152 & 104 & 56 & 39 & 244 & 1.334\\
 &SVC & 0 &  263 & 108 &  1 & 223 & 1.564\\ \hline\hline
 1.25&naive1 &  0 & 456 & 59 &24 & 56 & 1.25\\
 &naive2 & 301 & 43 & 12 & 10 & 229 & 0.96\\
 &naive3 & 282 & 70 & 32 & 26 & 185 & 0.95\\
 &SVC & 40 &  374 & 32 &  26 & 123 & 1.27\\ \hline\end{tabular}
  \caption{Online algorithm results for Bandwidth Profile 3}
  \label{tab:onlineReal}
\end{table}
 \begin{figure*}
\centering
\epsfig{file=figures/play_rate_svc_W_120_alpha_20_sf_4_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/play_rate_svc_W_120_alpha_20_sf_5_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/play_rate_svc_W_120_alpha_20_sf_6_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/play_rate_svc_W_120_alpha_20_sf_8_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\caption{Playback rate, online algorithm, and bandwidth profile (3)}
\label{fig:onlineResults}
\end{figure*}

 \subsubsection{Bandwidth profile 4}

  In the case of the average Bw of $2.5 Mb/s$, as shown in table () and figure(),  online SVC and naive 1 do not run into stalls. However, SVC has the highest average quality with $1.8$ and about $90\%$ of the frames are delivered in quality $\geq$ $1^{st}$ enhancement layer. Naive 1 delivers more than $50\%$ of the frames in a quality of the base layer. naive 2 and naive 3 do not deliver about $15\%$ of the frames. Bandwidth profile 2 and Average Bw of $1.8 Mb/s$.\\
In this specific scenario where the bandwidth starts very low even the average bandwidth is as high as 1.8, all algorithms run into stalls. As table () and figure () describes, naive 2 and 3 do not deliver about $30\%$ of the frames. Online SVC and naive 1 have the lowest number of stalls, and in average SVC deliver frames in higher quality than naive 1 with value of 1.382 and 1.23 for SVC and naive 1 respectively.

  \begin{table}
	\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Avg\_BW&Algo&\#stalls& \#b&\#e1&\#e2 &\#e3 &APBR\\ \hline
 2.5Mbps&naive1 &  0 & 356 & 83 & 21 & 135 & 1.41\\
 &naive2 & 93 & 48 & 21 & 17 & 416 & 1.687\\
 &naive3 & 86 & 43 & 35 & 64 & 367 & 1.687\\
 &SVC & 0 &  70 & 169 &  120 & 236 & 1.802\\ \hline\hline
 1.8Mbps&naive1 &  19 & 458 & 14 & 3 & 101 & 1.230\\
 &naive2 & 200 & 104 & 26 & 13 & 252 & 1.20\\
 &naive3 & 193 & 109 & 41 & 23 & 229 & 1.198\\
 &SVC & 12 &  345 & 91 &  17 & 130 & 1.382\\ \hline\hline
 1.5Mbps&naive1 &  250 & 263 & 26 & 5 & 51 & 0.74\\
 &naive2 & 362 & 66 & 17 & 15 & 135 & 0.695\\
 &naive3 & 361 & 68 & 17 & 21 & 128 & 0.692\\
 &SVC & 165 &  301 & 6 &  22 & 101 & 0.987\\ \hline\hline
 1.25&naive1 &  250 & 263 & 26 & 5 & 51 & 0.74\\
 &naive2 & 362 & 66 & 17 & 15 & 135 & 0.695\\
 &naive3 & 361 & 68 & 17 & 21 & 128 & 0.692\\
 &SVC & 165 &  301 & 6 &  22 & 101 & 0.987\\ \hline\end{tabular}
  \caption{Online algorithm results for Bandwidth Profile 4}
  \label{tab:onlineReal}
\end{table}
 \begin{figure*}
\centering
\epsfig{file=figures/bw_2_play_rate_svc_W_120_alpha_20_sf_4_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/bw_2_play_rate_svc_W_120_alpha_20_sf_5_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/bw_2_play_rate_svc_W_120_alpha_20_sf_6_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\epsfig{file=figures/bw_2_play_rate_svc_W_120_alpha_20_sf_9_z_600_5_startup_delay_vs_naive.eps, height=2in, width=3in}
\caption{Playback rate, online algorithm, and bandwidth profile (4)}
\label{fig:onlineResults}
\end{figure*}


==> useless.tex <==
\if 0

%We evaluate three variants of our algorithm. The first variant, SVC1, is a window-based algorithm with $W=60s$, $\alpha=20s$, chunk size = 1s, and $pe=25\%$. The second variant, SVC3, is perfect prediction over the entire video and uses a large chunk size of 60s to come up with large chunk policy which is then refined with a small chunk policy using a small chunk of 1s. The third variant, SVC2, refines SVC3 accounting for prediction errors. For large chunk,  the bandwidth profile with $50\%$ prediction error is used. Further, the refinement at the small chunk uses a window-based update with $\alpha=20$,  $W=60s$ where the bandwidth that is reserved for fetching later chunks is excluded, and a prediction error $pe=25\%$ is used for the small chunk.

%We highlight two findings.
%First, when the bandwidth is moderate, our scheme outperforms all three baseline schemes by fetching more EL3 chunks, leading to much higher overall playback bitrate. Second, in the low-bandwidth situation, all three of our schemes yield the smallest amount of skips compared to Baseline 2 and 3. However, all three of our schemes fetch lower number of chunks in base layer and has lower number of layer switches as compared to the Baseline 2 and Baseline 3. Baseline 1 is too conservative as it mostly fetches the base layer chunks while incurring a similar number of skipped chunks compared to our schemes do.


%three bandwidth profiles whose average bandwidth values are low (between BL and EL1), medium (between EL1 and EL2), and high (between EL2 and EL3), respectively.
%We use bandwidth profile 1 (Fig. \ref{fig : route}), and we scale it to simulate 3 different bandwidth regimes - low, moderate, and medium high.
%In the low regime, the average bandwidth is between $B$ and $E1$, while the moderate and the medium high cases have average bandwidth between $E1$ and $E2$, and between $E2$ and $E3$, respectively.

%The results in Fig \ref{fig : BComp} reveal that SVC1, SVC3, and SVC2 do not skip any chunk and get higher average quality  as compared to the  baselines which do not skip any chunk. Further, SVC2 performs almost the same as SVC3 thus depicting the robustness of the algorithm to prediction errors.

%Even though Baseline 2 fetches more chunks in $E3$ layer for medium high average bandwidth regime, it runs into stalls and  skips about $6\%$ of the chunks. In low and moderate regimes, we see that Baselines 2 and 3 skip more chunks ( about $20\%$ of the chunks in moderate regime, and about $45\%$ of the chunks for low regime). The reason behind not meeting the deadline of high percentage of chunks is the optimistic behavior of both algorithms (Baseline 2 and 3), where they fetch the next chunk in highest possible quality  without considering the future. In contrast, Baseline 1  is  conservative algorithm since it does not fetch chunks in $E1$ till all chunks are received in $B$ quality, and similar at higher layers. Even though Baseline 1 do not skip frames in medium high and moderate regimes, the average quality is low and so is the bandwith utilization. Our algorithms achieve the minimum number of stalls, and thus achieve the levels of the Baseline 1 in terms of skipped chunks. Among the baselines with least number of skipped chunks, SVCs achieve better average quality. Further, we have very few quality switches as compared to the baseline algorithms. We do not see any layer switch that jumps more than 1 level at a time as it is a case with optimistic algorithms (Baseline 2 and 3). In low regime,  SVC1 run into more stalls as compared to SVC3 and SVC2 which is expected since SVC uses prediction of only 1 minute ahead. Thus,  a coarse prediction of the future can be used to achieve better performance with the proposed algorithms.


%However, we see our algorithm do good job in avoiding stalls and fetching chunks in higher quality. It operates in a point that is between being very conservative and very optimistic. Both short and full path prediction based algorithms (SVC1 and SVC2) use prediction to decide the fetching policy that maintain high average and lowest number of stalls. Another point to notice, is that our algorithms have lowest number of layer switches among all. Especially, SVC2 algorithm since it uses the information of full prediction over the whole video period. The reason behind that is the priority that we give to later chunks when we solve the optimization problem in order to find the fetching policy. Moreover, we do not see any layer switch that jumps more than 1 level at a time as it is a case with optimistic algorithms (Baseline 2 and 3). In low regime, we see SVC1 run into more stalls than SVC2 and that is expected since it uses prediction of only 1 minute ahead. $\alpha$ and prioritizing later chunks help reducing the number of stalls though. %In all regimes, we see how close the policy of $SVC2$ to $SVC3$ which reflects the robust of our algorithm to the prediction error. We maintain the same average of the perfect prediction algorithm even we consider prediction errors of $50\%$ and $25\%$.


%The key take away messages that we can extract from Fig(\ref{fig : BComp}) are as following. First, from bar plots we clearly see that our both algorithms SVC1 and SVC2 maintain the highest playback average in all bandwidth regimes with compare to the all baseline algorithms. SVC2 is the closest to SVC3 (full path perfect prediction) which again reveals the truth that our algorithm is very robust to the prediction error as far as the predicted bandwidth is unbiased estimate of the real one.
 %it suffers from very low average fetching rate and low bandwidth utilization and it requires very large buffer.\\

%also shows breakdown of video chunks at different playback layers.
%
%
%But chunks at other layers are not much affected.

%	In conclusion, the change on the quality is not significant even though the change in the prediction error is very significant. Therefore, as far as the predicted bandwidth is unbiased estimator of the real one, we are not significantly deviated from the fetching policy of perfect prediction. This reflects the robustness of the algorithm to the prediction error. The reason behind not seeing significant effect of the prediction error is the prediction error adjustment that we use alongside the optimization.  Another thing to notice from the playback and the bandwidth profile figures, even though the bandwidth is high at the beginning and it gets lower later, we start to see chunks delivered in highest quality later on, and the reason behind that is that we give priority to later chunks when we maximize the number of chunks delivered in higher layers by setting $\gamma$ to some value $> 1$.

%In conclusion, our algorithm is robust to bandwidth prediction errors, thanks to the adjustment we use along with the optimization and the priority we give to later chunks in the optimization problem. Giving priority to later chunks helps having increased quality for later frames  which gives us increased time to fetch the higher quality later chunks.

%when we maximize the number of chunks delivered in higher layers by setting $\gamma$ to some value $> 1$.
%
%\shuai{how do we show support for the second point of setting $\gamma$ to some value $>1$?}
%When we set $\gamma$ to value $> 1$, we give priority to later chunks, and when we re-consider the decision every $\alpha$ we can change our decision and re-adjust to the bandwidth changes and bad prediction without loosing much since any decision of higher layers were made for later chunks.
%

%We also compare the window-based (online) scheme with the offline scheme where the bandwidth information for the entire playback period is perfectly known $(whole,0\%)$.

%We also simulate optimal case for performance comparison, and optimal means $(whole,0\%)$: perfect prediction is available for the whole period of the video.
%
%To better reflect real-life scenarios, we assumed higher prediction error for larger window size.
%by increasing $pe$ from 10\% to 25\% with step size of 5\% for the corresponding values of $W$.
%
%We also compare the window-based (online) scheme with the offline scheme where the bandwidth information for the entire playback period is perfectly known (\ie $W$ equals to the entire video duration and $pe$ equals to 0).
%To quantify the performance gap, we also ran the experiment with offline optimization, \ie $W$=125s, where 125 is the duration of fetching the video with perfect bandwidth prediction.
%

% First of all, from the bandwidth profile Fig(\ref{fig : wPlot}-a), we see the bandwidth is high at the beginning and it runs low later on. Small window sizes W=30-50 do not have enough prediction ahead to know that the bandwidth is low later on. Therefore, from the playback Fig(\ref{fig : wPlot}-b), we see the decision in the beginning is made to deliver some of the corresponding chunks in the $E1$ quality, and that cause skipping some chunks close to the end. However, from both playback and CDF figures Fig(\ref{fig : wPlot}-b) and Fig(\ref{fig : wPlot}-c), we notice that for W=50 we see less skips than W=40, and W=40 has less skips than W=30. The reason is two fold, First, we give higher priority to later chunks, and secondly we reconsider the decision of later chunks after $\alpha=15s$. For example for W=50, for first period we consider chunks from 1- 45 (50-startup delay +1). The decision would be final for chunks from 1 to 10 (15 -startup delay + 1). However, After 15s, we re-optimize for the chunks from (11- 51) over the time period (16 - 66). Therefore, there is a chance to re-consider the previous decision for the chunks 11-45 if they have not yet been fully fetched. Hence, we notice that for W=50, it drops the quality to the base layer early, after first policy re-consideration point, and it did not return to deliver chunks in E1 till the end. In other hand, we see for W=60, even though we have higher prediction error, we have exact match to the offline policy in CDF plot (same number of chunks fetched in every layer). The average fetching rates is almost same for all cases, 1.6521, 1.6771, 1.6646, 1.6667, 1.6667 for W=30, 40, 50, 60, and offline respectively.\\


 %Moreover, we consider our algorithm for scenario 2 where we firstly use large chunk size to have coarse grain policy and then convert it to small chunk size. The reason of the last one is to see how far this algorithm from the small chunk size policy. Later for long video where solving the optimization problem for small chunk becomes very expensive computationally, we will use this algorithm to integrate the low complexity of large chunk policy calculation with better performance of small chunk policy calculation.
%Fig \ref{fig : StoLchunkPlot} compares the cases when the chunk size is 1s, and 60s. More chunks in higher quality can be fetched with 1s chunk size because for 60s chunk policy, a decision of fetching a chunk in a certain layer has to be found for the whole 60s chunk. If the whole 60s chunk can be fetched in base layer quality but it can't be delivered in the $E1$ quality, then this chunk would be fetched in base layer quality. However, for 1s chunk size, the decision is more fined grained. a decision is taken for every 1s chunk. Therefore, even if there is a 60s segment that can't be fully fetched in $E1$ quality, some of its small sub chunks (1s chunks) can still be delivered in $E1$ quality. We see about $24\%$ of the chunks according to 1s policy calculation is delivered at $E1$ quality while all chunks according to $60s$ chunk policy calculation are delivered at base layer quality.

%Computational complexity forces us to use larger chunk size which gives a performance loss. In order to have a computationally efficient algorithm for large window sizes, we evaluate the proposed strategy with a large chunk of $60$s, and small chunk of $1$s. The computation uses entire video prediction for the large video and refines short chunk decisions using a window-based scheme  with $W=60$s, and $\alpha=30$s. We clearly see from the bar plot Fig( \ref{fig : StoLchunkPlot}(b) that the policy this  policy has the same number of chunks in every layer as the offline 1s chunk policy. In conclusion, calculating for large chunk, and then using small chunk decisions decreases computational complexity at the expense of some performance loss (which was zero in this example).

 % re-considering the decision every $\alpha$, and increasing the quality of later chunks if they are fetched earlier than their pre-decided fetching time help improving the large chunk decisions.




% We need to evaluate this improvement because we will use this algorithm for long video with reasonable coarse grain prediction of the bandwidth for the whole period of the video.
%In the case of long video with quite reasonable prediction of the bandwidth for the whole period of the video, solving the optimization program for small chunk size becomes very complex computationally. Therefore, using this strategy will integrate the low complexity of  large chunk based policy calculation with more fine grained decision of small chunk size.\\
% For comparison, we consider 1s chunk (offline), and we consider 60s chunk (offline) and then we re-consider the policy of 60s chunk every 30s for 1 minute ahead ($\alpha=30$, and $W=60$, online 60s-1s policy). If all chunks corresponding to the current window are fetched, we fetch the later chunks in the pre-decided quality. However, we increase their quality if they are fetched before a certain threshold less then the pre-decided fetching time.
 %We clearly see from the bar plot Fig( \ref{fig : StoLchunkPlot}-b) that the policy of online 60s -1s policy has the same number of chunks in every layer as the offline 1s chunk policy. It has improved the 60s chunk performance. %The playback figure Fig( \ref{fig : StoLchunkPlot}-a) shows there is some difference in the order of the chunks that are delivered at $E1$ quality, and the reason is that, when we re-consider the policy every 30s, we might've already delivered some chunks in higher quality since the priority is given to later chunks per window not the later chunk of the whole video as it is the case of offline 1s chunk policy.



% To evaluate the proposed no skip based streaming, we use the algorithms using SVC1, SVC3, and SVC2 described in the last section, with the adaptations for no skip based streaming described in Section \ref{sec:alg}. We compare the proposed algorithms to BBA-0 algorithm [], and Naive port of Microsoft's Smooth Streaming heuristic algorithm (NMS) []. We scale bandwidth profile 1 in low regime (Average bandwidth  of 3.09 Mbps) and medium high regime (Average bandwidth  of 7.19 Mbps). For BBA-0, we used the values for lower and upper threshold on the buffer  as $B_1=90$, and $B_m=216$, which are the values that were used in evaluating the algorithm in []. For NMS, we set lower buffer threshold $L=40\%$, upper threshold $U=70\%$, and panic threshold $P=25\%$ of the total buffer size. Moreover, for all algorithms we assume a  4 minutes long buffer. We note that in both the bandwidth regimes, SVC3 and SVC2 perform almost the same thus depicting robustness to error for our proposed algorithm.


%
%As shown, NMS suffer from high layer switching rates. This is due to its optimistic streaming
%strategies that blindly fetch high layers without considering potential bandwidth drop in the near future.
%
%Baseline 1, on the other hand, behaves very conservatively by first fetching the base layer for all chunks. Therefore it has low layer switching rates at the cost of low playback rates.
%
%We use moderate average bandwidth of 7.19Mbps (between EL2 and EL3) and low average bandwidth of 3.09Mbps (between BL and EL1), by appropriate scaling of bandwidth profile Fig. \ref{fig:route}. For a fair comparison with BBA-0 and NMS, the bit rates were chosen to be the same as corresponding encoding rates of SVC.

%Moreover, since BBA-0 is ABR based approach, we choose 4 different qualities Q1,Q2,Q3, and Q4, such that Q1=BL, Q2=EL1, Q3=EL2, and Q4=EL3.

%\shuai{We need to explain how we try to make fair comparison between SVC and ABR, since they are different technologies. \eg set ABR rates to be the same as corresponding encoding rates of SVC.}

%	To evaluate our no skip algorithm, we compared our algorithm both short prediction (pe=$25\%$) and full path based prediction $pe=50\%_25\%$ (SVC1 and SVC2) algorithms with the same parameters described in skip version simulation section with BBA-0 algorithm, and Naive port of Microsoft?s Smooth Streaming heuristic algorithm. We still use SVC3 (full path perfect prediction as a comparison reference ) %BBA0 is buffer based ABR algorithm (no prediction). It decides based on the buffer occupancy what quality should next chunk be delivered at. It starts fetching the chunks in the lowest quality up to a certain buffer occupancy (lower threshold) where it starts linearly increasing the quality of fetching with respect to the buffer occupancy , and it saturates at the highest quality level when it reaches the upper bound on the buffer occupancy (upper threshold). For more details about BBA0, the reader is referred to [].
%	For our comparison, we used bandwidth profile 1 in two regimes, high regime with average bandwidth (AvgBw=7.19mbps), and low regime with average bandwidth (AvgBW=3.09mbps).\\
	 %and the table Table.( \ref{tab : comp_ns}),

%In the moderate regime, we can see from Fig. \ref{fig:Comp_ns} that our  algorithms SVC1, SVC2 and SVC3 have the largest number of chunks played in higher qualities (with average quality of 6.8Mbps), followed by BBA-0  (5.8Mbps).
%
%NMS has the lowest average playback quality of 5.5Mbps.
%
%We also observe that BBA-0 does not fully utilize the available bandwidth, because it can only choose the lowest video quality before the buffer reaches $B_1$, which can happen either during the startup phase or when the buffer runs below $B_1$.
%
% NMS is also a buffer based approach and thus having loss in increasing quality while the aggressiveness in increasing the quality sooner increases the possibility that the buffer underruns later further increasing the cases where lower quality is fetched. The aggressiveness in switching to higher quality hurts the performance both in terms of average playback quality as well as larger layer switching rate.
%
%NMS is also a buffer based approach and thus suffers from a similar issue.
%
%We see from Fig. \ref{stall_comp_hiAvg.png}(b) that after about 25s, SVC1, SVC3, and SVC2 play most chunks in the highest quality level.
%
%In contrast, BBA-0  oscillates between layer E2 and E3, even though it starts fetching chunks in the highest quality level earlier than our algorithms.



%combines both buffer and bandwidth but since it does not use prediction and it aggressively increases the quality in the buffering state it runs in much higher layer switching rate and lower quality.
%From playback figure Fig.( \ref{stall_comp_hiAvg.png}-b), we can see after about 25s, SVC1 and SVC2 almost deliver all chunks in the highest quality level. In contrast to that we see BBA-0 still oscillating between $E2$ and $E3$ even though it did not start fetching chunks in the highest quality level earlier than our SVC1 and SVC2. The reason again is the buffer thresholding based fetching decision. NMS has the highest switching rate and in many cases it switches more than 1 quality level at a time which is very annoying to the user.\\

%In the low bandwidth regime, NMS has the largest stall period  (48s) and very high layer switching rate (we define layer switching rate as the number of jumps
%between \{BL,EL1\} and \{EL2,EL3\}.
%
%On the other hand, since BBA-0 is conservative, it performs well in terms of average quality.
%
%SVC1, SVC2, and BBA-0 have almost same average playback quality, 3.09Mbps, 3.06Mbps, and 3Mbps, respectively.
%
%However, compared to BBA, SVC2 plays very few chunks in base layer rate and has less frequent layer switches.
%
%\shuai{Anis: is the switch between base and higher layers or from higher to base layer?}
%
% Further, the number of layer switches between base and higher layers is very small for SVC2 as compared to BBA.
%
% SVC2 brings all stalls to the beginning using the knowledge of the bandwidth for the whole period. Thus, it has startup delay of about 15s (SVC3, perfect prediction, has startup delay of 12s). BBA-0, on the other hand,  has a startup delay of only 1s since it finds the startup delay based on the time needed to fetch one chunk in the base layer. However, it runs into 11 more seconds of stalls. Thus, the total stall time of the two algorithms is equivalent. SVC1 has higher duration of stalls (29 seconds) as compared to BBA-0 and SVC2. However,  it still offers higher average fetching rate than BBA-0. From the playback figure, we note that SVC1 has more stalls since it fetches earlier chunks at the highest quality based on the short prediction window and thus pays the penalty for the later chunks.
%
\iffalse
In terms of stalls, both SVC2 and BBA-0 have the same total stall duration of 12s.
%
But SVC2 brings all stalls to the beginning so that it is essentially part of the startup delay.
%
In this way, we can provide a much smoother video streaming experience with as little as possible stalls during the playback.
%
This is only possible because of our coarse grain prediction of future network bandwidth for the whole period with $pe=50\%$.
%
\shuai{This assumption seems too strong. Do we calculate the initial startup delay for SVC2 based on prediction for the whole trace? pe=?}
%
On the other hand, BBA-0 has a startup delay of only 1s since it finds the startup delay based on the time needed to fetch the first chunk in lowest rate.
%
However, it later runs into 11 more seconds of stalls, spread across the whole playback duration.


%the reason of running into more stalls for SVC1 is that it deliver some chunks in highest quality based on the short prediction window. Therefore, some later chunks would need more time to be fetched in the base layer according to the available bandwidth. However, this drawback can be avoided if we consider our algorithm SVC1 with buffer threshold that controls the number of higher enhancement layers we consider when we solve the optimization problem. In other words, if the average bandwidth is low and the buffer size is running low, we consider less number of enhancement layer when we solve the optimization problem. In both regimes, we see how close the policy of $SVC2$ to $SVC3$ which reflects the robust of our algorithm to the prediction error. We maintain the same average of the perfect prediction algorithm even we consider prediction errors of $50\%$ and $25\%$.


%Hence, even if we give BBA-0 a startup delay of 12s, we would still see it offering lower average fetching rate with compare to SVC2.

	%In low regime ; since NMS does not use prediction, and it relies on the current bandwidth and the buffer state, it experience the highest stall period  ($48s$) and very high layer switching rate. It jumps for more than 1 layer in one switch which is very annoying to the user. In the other hand, since BBA-0 is buffer based, it is expected that it would do good in low regime (conservative in low regime). Our algorithm SVC1, SVC2, and BBA-0 have very close average fetching rates with 3.1, 3.06, and 3Mbps respectively.
	
%	But SVC2 still win in term of fetching less chunks in base layer and maintaining lower layer switching rate and more stable delivery. SVC2, brings all stalls to the beginning using the knowledge of the bandwidth for the whole period; therefore, it has startup delay of about 15s (SVC3, perfect prediction, has startup delay of 12s), and. BBA-0 has startup delay of only 1s since it finds the startup delay based on the time enough to fetch one chunk in the base layer. However, it runs into 11 more seconds of stalls. Hence, even if we give BBA-0 a startup delay of 12s, we would still see it offering lower average fetching rate with compare to SVC2.

%SVC1 has higher stalls time than BBA-0 and SVC2. It runs into about 29 seconds of stalls, yet it still offer higher average fetching rate than BBA-0. From the playback figure, we can see that the reason of running into more stalls for SVC1 is that it deliver some chunks in highest quality based on the short prediction window. Therefore, some later chunks would need more time to be fetched in the base layer according to the available bandwidth. However, this drawback can be avoided if we consider our algorithm SVC1 with buffer threshold that controls the number of higher enhancement layers we consider when we solve the optimization problem. In other words, if the average bandwidth is low and the buffer size is running low, we consider less number of enhancement layer when we solve the optimization problem. In both regimes, we see how close the policy of $SVC2$ to $SVC3$ which reflects the robust of our algorithm to the prediction error. We maintain the same average of the perfect prediction algorithm even we consider prediction errors of $50\%$ and $25\%$.
	

\shuai{We need to double check numbers and texts after figures are finalized.}
%
We now demonstrate that the performance of our algorithms is not tied to the above chosen bandwidth profile.
%
We compare our algorithms (SVC1 and SVC2) with BBA-0 and NMS over three different profiles given in Fig.  \ref{fig:CompCDF_ns} for a 20-minute video.
%
All bandwidth profiles have average values in the moderate range (5-7Mbps).
%
We choose the moderate range because it is the most interesting scenario. %challenging range in term of making decisions for our algorithm.
%
We note that in all the bandwidth profiles except for bandwidth profile 2, all the algorithms can start playing back chunks with 1s startup delay without experiencing any interruptions.
%
However,  4s stall time is needed for all algorithms in the case of bandwidth profile 2.
%
SVC2 was able to bring this 4s stall time to the beginning as startup delay thanks to bandwidth prediction.
%
Further, Table \ref{tab:3pfComp} demonstrates that in all bandwidth profiles, SVC1 and SVC2 achieve the highest average quality and with the smallest number of chunks being fetched in base and EL1 layer.
%
SVC2 is the best in terms of minimum chunks obtained in lower qualities followed by SVC1.
%
Finally, we see that SVC2 maintains the lowest number of layer switching and thus has  more stable playback rate.

\fi
%	To show that our algorithm is not tight to single bandwidth profile, we compare our algorithm both short prediction (pe=$25\%$) and full path based prediction $pe=50\%_25\%$ (SVC1 and SVC2) with BBA-0 and NMS by simulate 6 of 20 minute video under 6 real collected bandwidth traces. We omit SVC3 results here in seek of space and since SVC2 has almost same results. The bandwidth traces as well as the comparison figures are shown in Fig.( \ref{fig:CompCDF_ns}).
%All bandwidth profiles have average values in the moderate range (5-7Mbps). We choose the moderate range because it is the most challenging range in term of making decisions. First, in all bandwidth profiles except bandwidth profile 5, all algorithms can start playing back chunks as early as 1s startup delay without experiencing interruptions. However, bandwidth profile 5 requires stall time of 4s for all algorithms. SVC2 was able to fetch all stalls to the beginning since it has full path prediction. Secondly, In all bandwidth profiles SVC1 and SVC2 has the highest average fetching rate (see table.\ref{tab : 6PfComp}) and the lowest number of chunks fetched in base layer and EL1 qualities. SVC2 comes in the $1^st$ place in term of minimizing number of chunks fetched in low quality, and then SVC1 comes in the $2^nd$. We see that even SVC1 uses short prediction (1 minute ahead), it uses it very efficiently by re-computing every $\alpha$ and prioritizing later chunks so it maintains the same average fetching rate of full path prediction. Finally, as the table ( \ref{tab : 6PfComp}) shows,  that SVC2 maintains the lowest number of layer switching and more stable delivery rate.

%	In this section we show how robust our algorithm to the prediction error. To evaluate our algorithm under prediction error, we simulated short video (2 minutes) over the bandwidth profile Fig(\ref{fig : peCdf}-a). This bandwidth profile is a small segment we cut from bandwidth profile 1 shown in Fig.(\ref{fig : route}). Moreover, we assume startup delay of 6s, and we set the chunk size to 1s. We assume prediction error of $0\%, 25\%, 50\%, 75\%$, and$100\%$. In all cases we assume unbiased bandwidth estimation . i.e, the real bandwidth could be higher or lower than the predicted one with equal probability.\\

% Table  \ref{tab : buffComp} and the CDF plot, Fig. \ref{fig : bufCdf}, of the quality clearly show as the buffer size increases, we see less stalls and more chunks delivered in higher layers. Looking into the CDF plot we see while about $30\%$ of the chunks are fetched in a quality of $E1$ or less for buffer size of 20MB, this percentage keep decreasing and the percentage of delivering in higher quality increases as the buffer size increases, so we see when the buffer size is 100MB, we have less than $10\%$ of the chunks are fetched in the $E1$, and the remaining $90\%$ of the chunks are fetched in higher quality levels.

%even though we have higher prediction error
% In conclusion, higher prediction window even with higher prediction error can take advantage of prioritizing later chunks and policy re-consideration every $\alpha$ and offer closer policy to the offline case. Short window size could run into the scenario where some chunks are delivered in higher quality but with the cost of that some others may not be fetched at all, and this can be clearly seen from the CDF plot Fig(\ref{fig : wPlot}-c) where we see more chunks are delivered in highest quality level when W=30 about $25\%$ of the chunks. However about $10\%$ of the chunks are not fetched at all.

%In conclusion, our algorithm can benefit from larger optimization window size $W,$ since that allows it to give higher priority to later chunks and rerun optimization more frequently. However, increasing $W$ has diminishing returns, this allowing us to get good gains with reasonable window sizes.
%

%Since base 1 is very conservative algorithm it is expected to have the lowest switching rate. Our online algorithm is trading off both high average rate and low switching rate and that is why we see the switching rate curve is some where in between. Another point to note is that shorter prediction comes with higher switching rate.

%For our algorithm, we use a buffer size of 4 minutes and a startup delay of 5s to ensure apple-to-apple comparison. We compare the performance of described algorithms on 50 traces of mobile dataset (HSDPA)~\cite{riiser2013commute} (The statistics are shown in Fig~\ref{fig : bwStat}.)

%Moreover we include offline, $(Whole,0\%)$ which is optimal for a given bandwidth profile, for comparison reason (i.e to see which online algorithm has closer performance to the theoretical upper bound).
%
%SVC1 is configured with $W=60s$, $\alpha=20s$, CS = 1s, and $pe=25\%$.
%SVC3 corresponds to perfect bandwidth prediction over the entire video and uses the two-phased optimization (\S\ref{sec:largesmall}) where the large and small chunk sizes are 60s and 1s, respectively.
%large chunk size of 60s to come up with large chunk policy which is then refined with a small chunk policy using a small chunk of 1s. \feng{TODO}
%SVC2 refines SVC3 by further taking into account the prediction errors.
%For large chunks, a prediction error of $pe=50\%$ is assumed.
%The refinement for small chunks uses an optimization window with $\alpha=20$,  $W=60s$, and $pe=25\%$.
%where the bandwidth that is reserved for fetching later chunks is excluded, and a prediction error $pe=25\%$ is used for the small chunk.

% We first evaluate the effect of the prediction error, the window size $W,$ the recalculation point $\alpha$, the chunk size,and the buffer size on our algorithm. Secondly, we compare it with baselines described in section	` \ref{simulation} over a long video (1 hour video).


%Delivering video frames as a continuous stream, so the end user can start watching the video in the highest possible quality is the ultimate goal of different video streaming and coding techniques. To achieve this goal, the available bandwidth should be used in the most efficient way.
%%The three fundamental challenges in video streaming are unknown and time-varying bandwidth, delay jitter, and loss[1].
%Therefore, different coding techniques were developed in order to adjust the delivered quality according to the available bandwidth. For example Adaptive bitrate (ABR) encodes the video into multiple bit rates corresponding to different qualities stored as different files and each file is partitioned into a sequence of small segments (chunks), and a decision to deliver specific chunk from which file (which quality level) is made based on the available bandwidth at the time of the delivery. In the other hand, Scalable Video Coding (SVC) encodes only a single file that is constructed from base layer (BL) and multiple enhancement layers (ELs). These sub streams can be encoded by exploiting three scalability features: (i) spatial scalability by layering image resolution (screen pixels) (ii) temporal scalability by layering the frame rate, and (iii) quality scalability by layering the image compression[].
%Therefore, in the limited bandwidth case, based on the available bandwidth, a decision is made on up to what enhancement layer a specific chunk can be delivered.  The base layer can be independently decoded, providing a base level of quality. Enhancement layers are decoded if and only if the base layer and all lower layers have been received and decoded. Therefore, the more ELs can be delivered, the better quality of the video stream is achieved. SVC benefits both content providers and end users since content providers need prepare only one high quality SVC-encoded video file and users request and fetch different numbers of layers to adapt their video bitrates based on their resource availability.
%
%In mobile video streaming, the available link capacity of a user may vary over time and space depending on its signal strength, other users traffic in the same cell, trajectory of user movement, and link condition variation. However, if the bandwidth can be predicted for sometime ahead, better decision on what chunk should be fetched at what quality level can be made. In general there are many scenarios where the bandwidth can be predicted. Even though the user scheduling decisions and channel states could change very rapidly, i.e  in scale of milliseconds, the average available bandwidth per user in scale of a chunk period, few seconds, still can be predicted and related to the expected signal strengths at different zones of the user trajectory and under different cell loads. Moreover, bandwidth profiles of other users who passed through the same zone on a given hour previously,  can be a unbiased estimate for the current profile.
%For example a user who is downloading a video and driving on a road that passes through different zones with different signal strengths under some cell load that would not dramatically changes in order of minutes would be known that he/she would most probably experience a certain bandwidth profile while he/she is moving.



%This bandwidth profile can be extracted using a crowd-sourced information using the bandwidth profiles of other users who travelled the same road recently. Monitoring user position, and speed can yield a good estimate on how the available bandwidth will vary over time, which can be refined further. Using such information of the future can lead to better predictive steaming algorithms, which is the focus of this work.

%long it would take the user to leave a zone and enter another, so the user bandwidth profile over time can be predicted, and it still can be corrected if the user drifts by increasing or decreasing the speed. Therefore, finding a way to pre-fetch as much as the buffer allow of later chunks when the bandwidth is high would minimize the probability of interruption later on, and finding a good strategy to decide which chunk should be fetched in what quality and what time based on the predicted bandwidth can maximize the number of chunks that can be fetched in higher enhancement layers. The policy could be re-calculated every few time units to adjust to the prediction error and profile if the user drifts from the previouslly predicted one.

%Moreover, at any given zone where multiple users entering and leaving the zone, and in scale of few minutes, the bandwidth profile of new user can be predicted based on that bandwidth profiles that were experienced by other users in the same zone since there would not be dramatic change in scale of few minutes. Therefore, if the bandwidth information can be collected from other users, the bandwidth profile of a new user can be predicted.

%	In this paper we propose an efficient algorithm to adaptively stream SVC videos with qualities being decided based on the predicted future bandwidth. We propose algorithm for skip version where user skips chunks that do not meet their deadlines as well as no-skip version where user watch every thing even if it takes him/her more time. For skip version streaming, the video is played with an initial start-up (i.e., buffering) delay and there is a deadline for each of the chunks. Chunks not received by the respective deadline are skipped. For no-skip, it also has start-up delay. However, if a chunk cannot be downloaded by its deadline, it will not be skipped. Instead, a stall will be incurred i.e., the video will pause before the chunk is fully downloaded. In both scenarios, the goal of the scheduling algorithm is to determine up to which layer we need to fetch for each chunk (except for those skipped in real-time streaming), such that the overall playback bitrate is maximized and the number of stalls or chunk skips is minimized. Moreover, we propose an algorithm to adjust to prediction error and change decisions on fly.
%To motivate the problem further let's assume a road or where users can cooperate by sharing the bandwidth that they experienced in different zones with each other. It is expected that at any zone in order of few minutes mostly there won't be dramatic change in the number of users and the environment. If a user left the zone, most probably another one will enter it. Therefore any set of entering users at any time will most probably experience the same average bandwidth per second the leaving set have experienced, and it is a matter of first few frames to decide the bandwidth profile of a certain user x entering the zone will be most probably same as another user y who just left the zone (see figure 2).\\
%\includegraphics{tunnelScenario.eps}
%\begin{figure*}
%\centering
%\epsfig{file=figures/bw_1_60.eps, height=2in, width=3in}
%\epsfig{file=figures/play_rate_svc_vs_abr.eps, height=2in, width=3in}
%\caption{SVC vs ABR (a) the bandwidth profile and (b) the playback rate}
%\label{fig:svcVsAbr}
%\end{figure*}

%Since we are relying on bandwidth prediction, and the prediction may not be perfect. i.e, real bandwidth could differ from the predicted one, SVC would be a reasonable choice. To explain why SVC is a good choice, assume a user is downloading a real time video where every chunk is needed to be either delivered within its deadline or skipped if it can't meet the deadline. Assume that based on the bandwidth prediction a decision was made to download a chunk $i$ in the quality of $j$th enhancement layer, ($BL + jELs$), at time period $t$ to $t+k$. Moreover, assume that $t+k$ is the deadline of the chunk, and the base layer and $m$ enhancement layers of the chunk were downloaded in the period between $t$ to $t+c$ where $c < k$ and $m < j$. However, the real bandwidth turns out to be less than the predicted one and the time from $c+1$ to $k$ is not enough to download the chunk in the pre-decided quality, so the user still can play the chunk on at least the $m$th enhancement layer quality. Compare this with what would happen if ABR was used and a choice was made to fetch the chunk on the $j$th quality. Since ABR choses one of pre-coded qualities, it can not change the decision on fly. Therefore, ABR would either exceed the deadline of the chunk or not completely fetch it before its deadline, so the playback would be interrupted and subsequent chunks would be affected.
%To further explore the advantage of SVC over ABR, we simulate a video with a length of 120s, using the bandwidth profile shown in figure (1). The average bandwidth is 1.7, and prediction error of $50\%$. Fig. \ref{fig:svcVsAbr} shows the advantage of using SVC over ABR. As shown in the figure, the real bandwidth was not enough to deliver the video frames at time 45 time slot and 58 time slot, so the ABR algorithm fails to deliver the frame while the SVC was able to deliver the frame in lower quality.


%This is the first work, to the best of our knowledge, that develop algorithms that explicitly and strategically leverage the future knowledge of network conditions for better performance using SVC encoding.


% The main contributions of the paper are as follows.
%
%\noindent 1. This paper propose a robust streaming algorithm for SVC video streaming. The variants of the algorithm are given for both the skip based streaming, where the chunks that are not played by the deadline are skipped (nothing is played in the stall duration, but the skipped chunk is not played in the future too) and the no-skip based streaming where each chunk is played, even if there are stalls. The proposed algorithm uses a set of linear optimization problems, which can be solveby any generic solver. The algorithms are adapted to window-based streaming  and are robust to  bandwidth prediction errors which are typical of cellular environments.
%
%\noindent 2. In order to reduce the computational complexity when the prediction window is large, we use a 2 -phase algorithm,  where an initial run uses large chunk sizes, and the output is then adapted to the case of smaller chunk sizes, thus decreasing the overall run time.
%
%\noindent 3. The algorithm  is shown to be robust to prediction errors, and works well with reasonable window sizes. Further, the algorithm is compared to several naive strategies for the skip version, and BBA-0 \cite{BBA} and the SVC version of Microsoft's smooth streaming algorithm\cite{SVCMetrics}. The simulation results depict the improved performance of the proposed algorithm in terms of metrics like the average quality, quality switching, number of skips or stalls. For moderate average bandwidth, the average  video quality using the proposed algorithm is 25\% better than \cite{BBA,SVCMetrics}.
%
%\noindent 4. In addition to the simulations, the proposed algorithm is also emulated using a testbed between a commodity laptop and a server inter-connected using high-speed Ethernet. The emulation results are very close to the simulation results further showing that the proposed algorithm is robust to the overheads of  TCP and other protocols.

%We formulate our decision process that determines for each portion of the video, how many of the layers to download, given network conditions), and which chunks can be as an optimization problem (to optimize desired QoE metrics like minimizing stalls and maximizing average playback bitrate etc.), We solve the offline problem optimally.

%\noindent 2. In order to reduce the computational complexity when the prediction window is large, we develop a two-phased approach, where an initial run of the original algorithm uses large chunk sizes. The output of this phase is then adapted to  smaller chunk sizes, thus significantly decreasing the overall run time with a minor decrease in the performance.


\fi

